Foundations of User-Centric Cell-Free Massive MIMO

Imagine a coverage area where each mobile device is communicating with a preferred set of wireless access points (among many) that are selected based on its needs and cooperate to jointly serve it, instead of creating autonomous cells. This effectively leads to a user-centric post-cellular network architecture, which can resolve many of the interference issues and service-quality variations that appear in cellular networks. This concept is called User-centric Cell-free Massive MIMO (multiple-input multiple-output) and has its roots in the intersection between three technology components: Massive MIMO, coordinated multipoint processing, and ultra-dense networks. The main challenge is to achieve the benefits of cell-free operation in a practically feasible way, with computational complexity and fronthaul requirements that are scalable to enable massively large networks with many mobile devices. This monograph covers the foundations of User-centric Cell-free Massive MIMO, starting from the motivation and mathematical definition. It continues by describing the state-of-the-art signal processing algorithms for channel estimation, uplink data reception, and downlink data transmission with either centralized or distributed implementation. The achievable spectral efficiency is mathematically derived and evaluated numerically using a running example that exposes the impact of various system parameters and algorithmic choices. The fundamental tradeoffs between communication performance, computational complexity, and fronthaul signaling requirements are thoroughly analyzed. Finally, the basic algorithms for pilot assignment, dynamic cooperation cluster formation, and power optimization are provided, while open problems related to these and other resource allocation problems are reviewed. All the numerical examples can be reproduced using the accompanying Matlab code.

==> NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> SIG-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{SIGcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {SIGcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Signal Processing}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SIG}
\journalurl        {http://www.nowpublishers.com/SIG}
\journalissnprint  {1932-8346}
\journalissnonline {1932-8354}
\journaldoi        {10.1561/20}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Signal Processing publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
\footnotesize
 \begin{itemize}
\item{Adaptive signal processing}
\item{Audio signal processing}
\item{Biological and biomedical signal processing}
\item{Complexity in signal processing}
\item{Digital signal processing}
\item{Distributed and network signal processing}
\item{Image and video processing}
\item{Linear and nonlinear filtering}
\item{Multidimensional signal processing}
\item{Multimodal signal processing}
\item{Multirate signal processing}
\item{Multiresolution signal processing}
\item{Nonlinear signal processing}
\item{Randomized algorithms in signal processing}
\item{Sensor and multiple source signal processing, source separation}
\item{Signal decompositions, subband and transform methods, sparse representations}
\item{Signal processing for communications}
\item{Signal processing for security and forensic analysis, biometric signal processing}
\item{Signal quantization, sampling, analog-to-digital conversion, coding and compression}
\item{Signal reconstruction, digital-to-analog conversion, enhancement, decoding and inverse problems}
\item{Speech/audio/image/video compression}
\item{Speech and spoken language processing}
\item{Statistical/machine learning}
\item{Statistical signal processing}
	\begin{itemize}
	\item{Classification and detection}
	\item{Estimation and regression}
	\item{Tree-structured methods}
	\end{itemize}
\end{itemize}
\normalsize
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Signal Processing, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> SIG-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Massive MIMO Networks: Spectral, Energy, and Hardware Efficiency}\\
Emil Bjornson, Jakob Hoydis and Luca Sanguinetti\\
ISBN: 978-1-68083-985-2\\
\\
\noindent \textit{Using Inertial Sensors for Position and Orientation Estimation}\\
Manon Kok, Jeroen D. Hol and Thomas B. Schon\\
ISBN: 978-1-68083-356-0\\
\\
\noindent \textit{Computational Visual Attention Models}\\
Milind S. Gide and Lina J. Karam\\
ISBN: 978-1-68083-280-8\\
\\
\noindent \textit{Video Coding: Part II of Fundamentals of Source and Video Coding}\\
Thomas Wiegand and Heiko Schwarz\\
ISBN: 978-1-68083-178-8

==> cell-free-book-nowbook.tex <==
\PassOptionsToClass {book,biber}{nowfnt}
\input {cell-free-book}


==> cell-free-book-nowchapter.tex <==
\PassOptionsToClass {chapter,biber}{nowfnt}
\input {cell-free-book}


==> cell-free-book-nowebook.tex <==
\PassOptionsToClass {ebook,biber}{nowfnt}
\input {cell-free-book}


==> cell-free-book-nowechapter.tex <==
\PassOptionsToClass {echapter,biber}{nowfnt}
\input {cell-free-book}


==> cell-free-book-nowplain.tex <==
\PassOptionsToClass {plain,biber}{nowfnt}
\input {cell-free-book}


==> cell-free-book-nowsample.tex <==
\PassOptionsToClass {sample,biber}{nowfnt}
\input {cell-free-book}


==> journaldata/ACC-editorialboard.tex <==
%ACC-Editorialboard.

\begin{editorialboard}

%\subsection{Editor-in-Chief}

%\journalchiefeditor{Stefan J. Reichelstein}{Stanford University\\United States}



\subsection{Executive Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Jonathan Glover, Editor-in-Chief}{Columbia University}
\journaleditor{Stephen Penman}{Columbia University}
\journaleditor{Stefan J. Reichelstein}{Stanford University and University of Mannheim}
\journaleditor{Dan Taylor}{University of Pennsylvania}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/ACC-journaldata.tex <==
 	\definecolor{officegreen}{rgb}{0.0, 0.5, 0.0}
\colorlet{ACCcolor}{officegreen}   %new color names can be defined before use
\journalcolor      {ACCcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Accounting}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ACC}
\journalurl        {http://www.nowpublishers.com/ACC}
\journalissnprint  {1554-0642}
\journalissnonline {1554-0650}
\journaldoi        {10.1561/14}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Accounting publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Auditing}
\item{Corporate Governance}
\item{Cost Management}
\item{Disclosure}
\item{Event Studies/Market Efficiency Studies}
\item{Executive Compensation}
\item{Financial Reporting}
\item{Management Control}
\item{Performance Measurement}
\item{Taxation}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Accounting, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ACC-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Foreign Currency: Accounting, Communication and Management of Risks}\\
Trevor Harris and Shiva Rajgopal\\
ISBN: 978-1-68083-946-3
\\
\\
\noindent \textit{Audit Regulations, Audit Market Structure, and Financial Reporting Quality}\\
Christopher Bleibtreu and Ulrike Stefani\\
ISBN: 978-1-68083-900-5
\\
\\
\noindent \textit{Accounting for Risk}\\
Stephen Penman\\
ISBN: 978-1-68083-890-9
\\
\\
\noindent \textit{Evolution of U.S. Regulation and the Standard-Setting Process for Financial Reporting: 1930s to the Present}\\
Stephen A. Zeff\\
ISBN: 978-1-68083-864-0
\\
\\
\noindent \textit{IFRS: Markets, Practice, and Politics}\\
Kirstin Becker, Jannis Bischof and Holger Daske\\
ISBN: 978-1-68083-830-5
\\
\\
\noindent \textit{Using Python for Text Analysis in Accounting Research}\\
Vic Anand, Khrystyna Bochkay, Roman Chychyla and Andrew Leone\\
ISBN: 978-1-68083-760-5



==> journaldata/ACG-editorialboard.tex <==
%ACG-Editorialboard.

\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Marc Goergen}{IE Business School\\Spain}
\journalchiefeditor{Geoffrey Wood}{Western University\\Canada}

\subsection{Founding Editor}

\editor{Douglas Cumming}{Florida Atlantic University, USA}

\subsection{Senior Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Renee Adams}{University of Oxford}
\journaleditor{Lucian Bebchuk}{Harvard University}
\journaleditor{William Judge}{Old Dominion University}
\journaleditor{Mark Roe}{Harvard University}
\journaleditor{Rene Stulz}{Ohio State University}
\journaleditor{James Westphal}{University of Michigan}
%\end{multicols*}

\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Amedeo de Cesari}{Alliance Manchester Business School}
\journaleditor{Patricia Gabaldon}{IE Business School}
\journaleditor{Aleksandra Gregoric}{Copenhagen Business School}
\journaleditor{Anna Grosman}{Loughborough University}
\journaleditor{Zulfiquer Haider}{Western University}
\journaleditor{Hang Le}{Nottingham Business School}
\journaleditor{Ben Sila}{Edinburgh University Business Schoo}
\journaleditor{Moshfique Uddin}{Leeds University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/ACG-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{ACGcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {ACGcolor} %a color name. 
\journaltitle      {Annals of Corporate Governance}
%\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ACG}
\journalurl        {http://www.nowpublishers.com/ACG}
\journalissnprint  {2381-6724}
\journalissnonline {2381-6732}
\journaldoi        {10.1561/109	}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
Annals of Corporate Governancepublishes
 articles in the following topics:
% \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Boards of Directors}
\item{Ownership}
\item{National Corporate Governance Mechanisms}
\item{Comparative Corporate Governance Systems}
\item{Self Governance}
\item{Teaching Corporate Governance}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
 Annals of Corporate Governance, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ACG-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Enterprise Foundations: Law, Taxation, Governance, and Performance}\\
Steen Thomsen and Nikolaos Kavadis
\\ISBN: 978-1-68083-942-5
\\
\noindent \textit{Beyond ESG: Reforming Capitalism and Social Democracy}\\
Marcel Boyer
\\ISBN: 978-1-68083-894-7
\\
\noindent \textit{The Social Purpose of the Modern Business Corporation}\\
Peter J. Buckley
\\ISBN: 978-1-68083-874-9
\\
\noindent \textit{Decentralized Autonomous Organizations: Internal Governance and External Legal Design}\\
Wulf A. Kaal
\\ISBN: 978-1-68083-798-8
\\
\noindent \textit{Decentralized Corporate Governance via Blockchain Technology}\\
Wulf A. Kaal
\\ISBN: 978-1-68083-676-9



==> journaldata/ASTP-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Albert N. Link}{University of North Carolina at Greensboro\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{David Audretsch}{Indiana University}
\journaleditor{William Bonvillian}{MIT}
\journaleditor{Barry Bozeman}{Arizona State University}
\journaleditor{Kaye Husbands Fealing}{Georgia Institute of Technology}
\journaleditor{John Hardin}{North Carolina Board of Science and Technology}
\journaleditor{Mariagrazia Squicciarini}{OECD}
\journaleditor{Wolfgang Polt}{Joanneum Research Institute}
\journaleditor{Nicholas Vonortas}{The George Washington University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/ASTP-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{ASTPcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {ASTPcolor} %a color name. 
\journaltitle      {Annals of Science and Technology Policy}
%\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ASTP}
\journalurl        {http://www.nowpublishers.com/ASTP}
\journalissnprint  {2475-1820}
\journalissnonline {2475-1812}
\journaldoi        {10.1561/110}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Annals of Science and Technology Policy publishes
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Literature reviews of technology and innovation policies}
\item{Historical case studies of technology development and implementation}
\item{Institutional histories of technology- and innovation-based organizations}
\item{Analyses of policies attendant to technology development and adoption and diffusion}
\item{Studies documenting the adoption and diffusion of technologies and subsequent consequences}
\item{Studies of public and private research partnerships (cross sectional, over time, or case based)}
\item{Assessments and evaluations of specific technology and innovation policies}
\item{Analyses of ecosystems associated with the technology and/or innovation development}
\item{Cross observational (e.g., cross-agency or cross-country) comparisons of technology and innovation policies}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
  Annals of Science and Technology Policy, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ASTP-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Government Royalties on Sales of Pharmaceutical and Other Biomedical Products Developed with Substantial Public Funding: Illustrated with the Technology Transfer of the Drug-Eluting Coronary Stent}\\
Robert S. Danziger and John T. Scott\\
ISBN: 978-1-68083-820-6\\

\noindent \textit{Case Studies of Successful Technology Transfer from Federal Laboratories}\\
Gretchen B. Jordan, Christopher S. Hayter, Michael Hogan, Manuel A. Gonzalez and Alan C. O’Connor\\
ISBN: 978-1-68083-808-4\\

\noindent \textit{Toward More Effective Science and Technology Advice for Congress: The Historical Roots and Pathways Forward}\\
Peter D. Blair\\
ISBN: 978-1-68083-802-2\\

\noindent \textit{The Globalization of the Bayh–Dole Act}\\
Thorsten Gores and Albert N. Link\\
ISBN: 978-1-68083-754-4\\

\noindent \textit{Globalization and the High-Tech Policy Response}\\
Gregory Tassey\\
ISBN: 978-1-68083-690-5\\
\\
\noindent \textit{Evolution of Ireland’s Industrial, Science and Technology Policy}\\
James A. Cunningham, Patrick Collins and Majella Giblin\\
ISBN: 978-1-68083-680-6\\
\\


==> journaldata/CGV-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

%\begin{multicols*}{2}\raggedcolumns
\journalchiefeditor{Aaron Hertzmann }{Adobe Research, USA}
%\end{multicols*}


\subsection{Editors} \scriptsize
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Marc Alexa}{TU Berlin}
\journaleditor{Kavita Bala}{Cornel}
\journaleditor{Ronen Basri}{Weizmann Institute of Science}
\journaleditor{Peter Belhumeur}{Columbia University}
\journaleditor{Andrew Blake}{Microsoft Research}
\journaleditor{Chris Bregler}{Facebook-Oculus}
\journaleditor{Joachim Buhmann}{ETH Zurich}
\journaleditor{Michael Cohen}{Facebook}
\journaleditor{Brian Curless}{University of Washington}
\journaleditor{Paul Debevec}{USC Institute for Creative Technologies}
\journaleditor{Julie Dorsey}{Yale}
\journaleditor{Fredo Durand}{MIT}
\journaleditor{Olivier Faugeras}{INRIA}
\journaleditor{Rob Fergus}{NYU}
%\columnbreak
\journaleditor{William T. Freeman}{MIT}
\journaleditor{Mike Gleicher}{University of Wisconsin}
\journaleditor{Richard Hartley}{Australian National University}
\journaleditor{Hugues Hoppe}{Microsoft Research}
\journaleditor{C. Karen Liu}{Stanford}
\journaleditor{David Lowe}{University of British Columbia}
\journaleditor{Jitendra Malik}{ Berkeley}
\journaleditor{Steve Marschner}{Cornell}
\journaleditor{Shree Nayar}{Columbia}
\journaleditor{Tomas Pajdla}{Czech Technical University}
\journaleditor{Pietro Perona}{California Institute of Technology}
\journaleditor{Marc Pollefeys}{ETH Zurich}
%\columnbreak
\journaleditor{Jean Ponce}{Ecole Normale Superieure}
\journaleditor{Long Quan}{HKUST}
\journaleditor{Cordelia Schmid}{INRIA}
\journaleditor{Steve Seitz}{University of Washington}
\journaleditor{Amnon Shashua}{Hebrew University}
\journaleditor{Peter Shirley}{University of Utah}
\journaleditor{Noah Snavely}{Cornell}
\journaleditor{Stefano Soatto}{UCLA}
\journaleditor{Richard Szeliski}{Microsoft Research}
\journaleditor{Luc Van Gool}{KU Leuven and ETH Zurich}
\journaleditor{Joachim Weickert}{Saarland University}
\journaleditor{Song Chun Zhu}{UCLA}
\journaleditor{Andrew Zisserman}{Oxford}
\end{multicols*}
\end{editorialboard} 

==> journaldata/CGV-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{CGVcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {CGVcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Computer Graphics and Vision}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {CGV}
\journalurl        {http://www.nowpublishers.com/CGV}
\journalissnprint  {1572-2740}
\journalissnonline {1572-2759}
\journaldoi        {10.1561/06}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Computer Graphics and Vision publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Rendering}
\item{Shape}
\item{Mesh simplification}
\item{Animation}
\item{Sensors and sensing}
\item{Image restoration and enhancement}
\item{Segmentation and grouping}
\item{Feature detection and selection}
\item{Color processing}
\item{Texture analysis and synthesis}
\item{Illumination and reflectance modeling}
\item{Shape representation}
\item{Tracking}
\item{Calibration}
\item{Structure from motion}
\item{Motion estimation and registration}
\item{Stereo matching and reconstruction}
\item{3D reconstruction and image-based modeling}
\item{Learning and statistical methods}
\item{Appearance-based matching}
\item{Object and scene recognition}
\item{Face detection and recognition}
\item{Activity and gesture recognition}
\item{Image and video retrieval}
\item{Video analysis and event recognition}
\item{Medical image analysis}
\item{Robot localization and navigation}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Computer Graphics and Vision, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/CGV-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Deep Learning for Multimedia Forensics}\\
Irene Amerini, Aris Anagnostopoulos, Luca Maiano and Lorenzo Ricciardi Celsi\\
ISBN: 978-1-68083-854-1\\
\\
\noindent \textit{Computer Vision for Autonomous Vehicles: Problems, Datasets and State of the Art}\\
Joel Janai, Fatma Güney, Aseem Behl and Andreas Geiger\\
ISBN: 978-1-68083-688-2\\
\\
\noindent \textit{Discrete Graphical Models - An Optimization Perspective}\\
Bogdan Savchynskyy\\
ISBN: 978-1-68083-638-7\\
\\
\noindent \textit{Line Drawings from 3D Models: A Tutorial}\\
Pierre Bénard and Aaron Hertzmann\\
ISBN: 978-1-68083-590-8\\
\\
\noindent \textit{Publishing and Consuming 3D Content on the Web: A Survey}\\
Marco Potenziani, Marco Callieri, Matteo Dellepiane and Roberto Scopigno\\
ISBN: 978-1-68083-536-6\\
\\
\noindent \textit{Crowdsourcing in Computer Vision}\\
Adriana Kovashka, Olga Russakovsky, Li Fei-Fei and Kristen Grauman\\
ISBN: 978-1-68083-212-9\\


==> journaldata/CIT-editorialboard.tex <==
\begin{editorialboard}

%\subsection{Editor-in-Chief}

\journalchiefeditor{Alexander Barg}{University of Maryland\\USA}

\subsection{Area Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Emmanuel Abbe}{Princeton University}
\journaleditor{Arya Mazumdar}{UMass Amherst}
\journaleditor{Olgica Milenkovic}{University of Illinois, Urbana-Champaign}
\journaleditor{Anelia Somekh-Baruch}{Bar-Ilan University}
\journaleditor{Himanshu Tyagi}{Indian Institute of Science}

\subsection{Editors} %\scriptsize
%\begin{multicols*}{3}\raggedcolumns
\journaleditor{Venkat Anantharam}{UC Berkeley}
\journaleditor{Giuseppe Caire}{TU Berlin}
\journaleditor{Daniel Costello}{University of Notre Dame}
%\journaleditor{Anthony Ephremides}{University of Maryland}
%\journaleditor{Andrea Goldsmith}{Stanford University}
\journaleditor{Albert Guillen i Fabregas}{Pompeu Fabra University}
\journaleditor{Dongning Guo}{Northwestern University}
\journaleditor{Dave Forney}{MIT}
\journaleditor{Te Sun Han}{University of Tokyo}
\journaleditor{Babak Hassibi}{Caltech}
\journaleditor{Michael Honig}{Northwestern University}
%\journaleditor{Tara Javidi}{UC San Diego}

\journaleditor{Ioannis Kontoyiannis}{Cambridge University}
\journaleditor{Gerhard Kramer}{TU Munich}
\journaleditor{Amos Lapidoth}{ETH Zurich}
\journaleditor{Muriel Medard}{MIT}
\journaleditor{Neri Merhav}{Technion}
\journaleditor{David Neuhoff}{University of Michigan}
\journaleditor{Alon Orlitsky}{UC San Diego}
\journaleditor{Yury Polyanskiy}{MIT}
\journaleditor{Vincent Poor}{Princeton University}
%\journaleditor{Maxim Raginsky}{UIUC}
\journaleditor{Kannan Ramchandran}{UC Berkeley}
\journaleditor{Igal Sason}{Technion}
%\columnbreak
\journaleditor{Shlomo Shamai}{Technion}
\journaleditor{Amin Shokrollahi}{EPF Lausanne}
\journaleditor{Yossef Steinberg}{Technion}
\journaleditor{Wojciech Szpankowski}{Purdue University}
\journaleditor{David Tse}{Stanford University}
\journaleditor{Antonia Tulino}{Bell Labs}
\journaleditor{R\"{u}diger Urbanke}{EPF Lausanne}
\journaleditor{Emanuele Viterbo}{Monash University}
\journaleditor{Frans Willems}{TU Eindhoven}
\journaleditor{Raymond Yeung}{CUHK}
\journaleditor{Bin Yu}{UC Berkeley}
\end{multicols*}
\end{editorialboard} 

==> journaldata/CIT-journaldata.tex <==
 	\definecolor{officegreen}{rgb}{0.0, 0.5, 0.0}
\colorlet{CITcolor}{officegreen}   %new color names can be defined before use
\journalcolor      {CITcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Communications and Information Theory}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {CIT}
\journalurl        {http://www.nowpublishers.com/CIT}
\journalissnprint  {1567-2190}
\journalissnonline {1567-2328 }
\journaldoi        {10.1561/01}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Communications and Information Theory publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Coded modulation}
\item{Coding theory and practice}
\item{Communication complexity}
\item{Communication system design}
\item{Cryptology and data security}
\item{Data compression}
\item{Data networks}
\item{Demodulation and Equalization}
\item{Denoising}
\item{Detection and estimation}
\item{Information theory and statistics}
\item{Information theory and computer science}
\item{Joint source/channel coding}
\item{Modulation and signal design}
\item{Multiuser detection}
\item{Multiuser information theory}
\item{Optical communication channels}
\item{Pattern recognition and learning}
\item{Quantization}
\item{Quantum information processing}
\item{Rate-distortion theory}
\item{Shannon theory}
\item{Signal processing for communications}
\item{Source coding}
\item{Storage and recording codes}
\item{Speech and Image Compression}
\item{Wireless Communications}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Communications and Information Theory, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/CIT-seriespage.tex <==
\vspace{12pt}
\\
\noindent \textit{Rank-Metric Codes and Their Applications}\\
Hannes Bartz, Lukas Holzbaur, Hedongliang Liu, Sven Puchinger, Julian Renner and Antonia Wachter-Zeh\\
ISBN: 978-1-63828-000-2\\
\\
\\
\noindent \textit{Common Information, Noise Stability, and Their Extensions}\\
Lei Yu and Vincent Y. F. Tan\\
ISBN: 978-1-63828-014-9\\
\\
\\
\noindent \textit{Information-Theoretic Foundations of DNA Data Storage}\\
Ilan Shomorony and Reinhard Heckel\\
ISBN: 978-1-68083-956-2\\
\\
\\
\noindent \textit{Asymptotic Frame Theory for Analog Coding}\\
Marina Haikin, Matan Gavish, Dustin G. Mixon and Ram Zamir\\
ISBN: 978-1-68083-908-1\\
\\
\noindent \textit{Modeling and Optimization of Latency in Erasure-coded Storage Systems}\\
Vaneet Aggarwal and Tian Lan\\
ISBN: 978-1-68083-842-8\\
\\
\noindent \textit{An Algebraic and Probabilistic Framework for Network Information Theory}\\
S. Sandeep Pradhan, Arun Padakandla and Farhad Shirani\\
ISBN: 978-1-68083-766-7\\




==> journaldata/DBS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Joseph M. Hellerstein}{University of California at Berkeley\\United States}
\journalchiefeditor{Surajit Chaudhuri}{Microsoft Research, Redmond\\United States}



\subsection{Editors} %\scriptsize
%\begin{multicols*}{3}\raggedcolumns
\journaleditor{Azza Abouzied}{NYU-Abu Dhabi}
\journaleditor{Gustavo Alonso}{ETH Zurich}
\journaleditor{Mike Cafarella}{University of Michigan}
\journaleditor{Alan Fekete}{University of Sydney}
\journaleditor{Ihab Ilyas}{University of Waterloo}
\journaleditor{Sunita Sarawagi}{IIT Bombay}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/DBS-journaldata.tex <==
 	\definecolor{officegreen}{rgb}{0.0, 0.5, 0.0}
\colorlet{DBScolor}{officegreen}   %new color names can be defined before use
\journalcolor      {DBScolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Databases}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {DBS}
\journalurl        {http://www.nowpublishers.com/DBS}
\journalissnprint  {1931-7883}
\journalissnonline {1931-7891}
\journaldoi        {10.1561/19}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Databases publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Data Models and Query Languages}
    \item{Query Processing and Optimization}
    \item{Storage, Access Methods, and Indexing}
    \item{Transaction Management, Concurrency Control and Recovery}
    \item{Deductive Databases}
    \item{Parallel and Distributed Database Systems}
    \item{Database Design and Tuning}
    \item{Metadata Management}
    \item{Object Management}
    \item{Trigger Processing and Active Databases}
    \item{Data Mining and OLAP}
    \item{Approximate and Interactive Query Processing}
    \item{Data Warehousing}
    \item{Adaptive Query Processing}
    \item{Data Stream Management}
    \item{Search and Query Integration}
    \item{XML and Semi-Structured Data}
    \item{Web Services and Middleware}
    \item{Data Integration and Exchange}
    \item{Private and Secure Data Management}
    \item{Peer-to-Peer, Sensornet and Mobile Data Management}
    \item{Scientific and Spatial Data Management}
    \item{Data Brokering and Publish/Subscribe}
    \item{Data Cleaning and Information Extraction}
    \item{Probabilistic Data Management}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Databases, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/DBS-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Natural Language Interfaces to Data}\\
Abdul Quamar, Vasilis Efthymiou, Chuan Lei and Fatma Özcan\\
ISBN: 978-1-63828-028-6\\
\\
\noindent \textit{Trends in Explanations: Understanding and Debugging Data-driven Systems}\\
Boris Glavic, Alexandra Meliou and Sudeepa Roy\\
ISBN: 978-1-68083-880-0\\
\\
\noindent \textit{Differential Privacy for Databases}\\
Joseph P. Near and Xi He\\
ISBN: 978-1-68083-850-3\\
\\
\noindent \textit{Database Systems on GPUs}\\
Johns Paul, Shengliang Lu and Bingsheng He\\
ISBN: 978-1-68083-848-0\\
\\
\noindent \textit{Machine Knowledge: Creation and Curation of Comprehensive Knowledge Bases}\\
Gerhard Weikum, Xin Luna Dong, Simon Razniewski and Fabian Suchanek\\
ISBN: 978-1-68083-836-7\\
\\
\noindent \textit{Cloud Data Services: Workloads, Architectures and Multi-Tenancy}\\
Vivek Narasayya and Surajit Chaudhuri\\
ISBN: 978-1-68083-774-2\\



==> journaldata/ECO-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{William H. Greene}{New York University\\United States}


\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Manuel Arellano}{CEMFI Spain}
\journaleditor{Wiji Arulampalam}{University of Warwick}
\journaleditor{Orley Ashenfelter}{Princeton University}
\journaleditor{Jushan Bai}{Columbia University}
\journaleditor{Badi Baltagi}{Syracuse University}
\journaleditor{Anil Bera}{University of Illinois}
\journaleditor{Tim Bollerslev}{Duke University}
\journaleditor{David Brownstone}{UC Irvine}
\journaleditor{Xiaohong Chen}{Yale University}
\journaleditor{Steven Durlauf}{University of Chicago}
\journaleditor{Amos Golan}{American University}
\journaleditor{Bill Griffiths}{University of Melbourne}
\journaleditor{James Heckman}{University of Chicago}
\journaleditor{Jan Kiviet}{University of Amsterdam}
\journaleditor{Gary Koop}{The University of Strathclyde}
\journaleditor{Michael Lechner}{University of St. Gallen}
\journaleditor{Lung-Fei Lee}{Ohio State University}
\journaleditor{Larry Marsh}{Notre Dame University}
\journaleditor{James MacKinnon}{Queens University}
\journaleditor{Bruce McCullough}{Drexel University}
\journaleditor{Jeff Simonoff}{New York University}
\journaleditor{Joseph Terza}{Purdue University}
\journaleditor{Ken Train}{UC Berkeley}
\journaleditor{Pravin Trivedi}{Indiana University}
\journaleditor{Adonis Yatchew}{University of Toronto}
\end{multicols*}
\end{editorialboard} 

==> journaldata/ECO-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{ECOcolor}{brickred}   %new color names can be defined before use
\journalcolor      {ECOcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Econometrics}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ECO}
\journalurl        {http://www.nowpublishers.com/ECO}
\journalissnprint  {1551-3076}
\journalissnonline {1551-3084}
\journaldoi        {10.1561/08}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Econometrics publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Econometric Models}
    \item{Simultaneous Equation Models}
    \item{Estimation Frameworks}
    \item{Biased Estimation}
    \item{Computational Problems}
    \item{Microeconometrics}
    \item{Treatment Modeling}
    \item{Discrete Choice Modeling}
    \item{Models for Count Data}
    \item{Duration Models}
   \item{Limited Dependent Variables}
    \item{Panel Data}
    \item{Time Series Analysis}
    \item{Latent Variable Models}
    \item{Qualitative Response Models}
    \item{Hypothesis Testing}
    \item{Econometric Theory}
    \item{Financial Econometrics}
    \item{Measurement Error in Survey Data}
    \item{Productivity Measurement and Analysis}
    \item{Semiparametric and Nonparametric Estimation}
    \item{Bootstrap Methods}
    \item{Nonstationary Time Series}
    \item{Robust Estimation}
\end{itemize}
 \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Econometrics, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ECO-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Performance Analysis: Economic Foundations and Trends}\\
Valentin Zelenyuk\\
ISBN: 978-1-68083-866-4\\
\\
\noindent \textit{Experimetrics: A Survey}\\
Peter G. Moffatt\\
ISBN: 978-1-68083-792-6\\
\\
\noindent \textit{Climate Econometrics: An Overview}\\
Jennifer L. Castle and David F. Hendry\\
ISBN: 978-1-68083-708-7\\
\\
\noindent \textit{Foundations of Stated Preference Elicitation: Consumer Behavior\\ and Choice-based Conjoint Analysis}\\
Moshe Ben-Akiva, Daniel McFadden and Kenneth Train\\
ISBN: 978-1-68083-526-7\\
\\
\noindent \textit{Structural Econometrics of Auctions: A Review}\\
Matthew L. Gentry, Timothy P. Hubbard, Denis Nekipelov and\\ Harry J. Paarsch\\
ISBN: 978-1-68083-446-8\\



==> journaldata/EDA-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Axel Jantsch}{TU Wien, Austria}


\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Bashir Al-Hashimi}{King's College London}
\journaleditor{Jason Cong}{University of California, Los Angeles}
\journaleditor{Christoph Grimm}{TU Kaiserslautern}
\journaleditor{Ahmed Jerraya}{CEA-Leti}
\journaleditor{Wolfgang Müller}{University of Paderborn}
\journaleditor{Partha Pande}{Washington State University}
\journaleditor{Zebo Peng}{Linköping University}
\columnbreak
\journaleditor{Christian Pilato}{Politecnico di Milano}
\journaleditor{Jaan Raik}{Tallinn University of Technology}
\journaleditor{Alberto Sangiovanni-Vincentelli}{University of California, Berkeley}
\journaleditor{Rishad Shafik}{Newcastle University}
\journaleditor{Sandeep Shukla}{Indian Institute of Technology, Kanpur}
\journaleditor{Norbert Wehn}{University of Kaiserslautern}
\end{multicols*}
\end{editorialboard} 

\subsection{Former Editors-in-chief}

\journaleditor{Sharad Malik}{Princeton University}
\journaleditor{Radu Marculescu}{The University of Texas at Austin}

==> journaldata/EDA-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{EDAcolor}{brickred}   %new color names can be defined before use
\journalcolor      {EDAcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Electronic Design Automation}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {EDA}
\journalurl        {http://www.nowpublishers.com/EDA}
\journalissnprint  {1551-3939}
\journalissnonline {1551-3947}
\journaldoi        {10.1561/10}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Electronic Design Automation publishes
 survey and tutorial articles in the following topics: 
%\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{System Level Design}
    \item{Behavioral Synthesis}
    \item{Logic Design}
    \item{Verification}
    \item{Test}
    \item{Physical Design}
    \item{Circuit Level Design}
    \item{Reconfigurable Systems}
    \item{Analog Design}
    \item{Embedded software and parallel programming}
   \item{Multicore, GPU, FPGA, and heterogeneous systems}
    \item{Distributed, networked embedded systems}
    \item{Real-time and cyberphysical systems}
\end{itemize}
% \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Electronic Design Automation, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/EDA-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Smart Healthcare}\\
Hongxu Yin, Ayten Ozge Akmandor, Arsalan Mosenia and Niraj K. Jha\\
ISBN: 978-1-68083-440-6\\
\\
\noindent \textit{Contracts for System Design}\\
Albert Benveniste, Benoit Caillaud, Dejan Nickovic, Roberto Passerone, Jean-Baptiste Raclet, Philipp Reinkemeier, Alberto Sangiovanni-Vincentelli, Werner Damm, Thomas A. Henzinger and Kim G. Larsen\\
ISBN: 978-1-68083-402-4\\
\\
\noindent \textit{Non-Boolean Computing with Spintronic Devices}\\
Kawsher A. Roxy and Sanjukta Bhanja\\
ISBN: 978-1-68083-362-1

==> journaldata/EES-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Marija D. Ili\'c}{MIT and Carnegie Mellon University\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{David Hill}{University of Hong Kong and University of Sydney}
\journaleditor{Rupamathi Jaddivadal}{SmartGridz}
\journaleditor{Daniel Kirschen}{University of Washington}
\journaleditor{J. Zico Kolter}{Carnegie Mellon University}
\journaleditor{Chao Lu}{Tsinghua University}
\journaleditor{Steven Low}{California Institute of Technology}
\journaleditor{Masoud H. Nazaril}{Wayne State University}
\journaleditor{Ram Rajagopa}{Stanford University}
\journaleditor{Lou van der Sluis}{TU Delft}
\journaleditor{Goran Strbac}{Imperial College London}
\journaleditor{Robert J. Thomas}{Cornell University}
\journaleditor{David Tse}{University of California, Berkeley}
\journaleditor{Le Xie}{Texas A\&M University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/EES-journaldata.tex <==
\definecolor{cinnabar}{rgb}{0.89, 0.26, 0.2}
\colorlet{EEScolor}{cinnabar}   %new color names can be defined before use
\journalcolor      {EEScolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Electric Energy Systems}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {EES}
\journalurl        {http://www.nowpublishers.com/EES}
\journalissnprint  {2332-6557}
\journalissnonline {2332-6565}
\journaldoi        {10.1561/31}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Electric Energy Systems publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Advances in power dispatch}
\item{Demand-side and grid scale data analytics}
\item{Design and optimization of electric services}
\item{Distributed control and optimization of distribution networks}
\item{Distributed sensing for the grid}
\item{Distribution systems}
\item{Fault location and service restoration}
\item{Integration of physics-based and data-driven modeling of future electric energy systems}
\item{Integration of Power electronics, Networked FACTS}
\item{Integration of renewable energy sources}
\item{Interdependence of power system operations and planning and the electricity markets}
\item{Microgrids}
\item{Modern grid architecture}
\item{Power system analysis and computing}
\item{Power system dynamics}
\item{Power system operation}
\item{Power system planning}
\item{Power system reliability}
\item{Power system transients}
\item{Security and privacy}
\item{Stability and control for the whole multi-layer (granulated) network with new load models (to include storage, DR, EVs) and new generation}
\item{System protection and control}
\item{The new stability guidelines and control structures for supporting high penetration of renewables (>50\%)}
\item{Uncertainty quantification for the grid}
\item{System impacts of HVDC}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
 Electric Energy Systems, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/EES-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Network-Based Analysis of Rotor Angle Stability of Power Systems}\\
Yue Song, David J. Hill and Tao Liu\\
ISBN: 978-1-68083-778-0\\
\\
\noindent \textit{A Survey of Relaxations and Approximations of the Power Flow Equations}\\
Daniel K. Molzahn and Ian A. Hiskens\\
ISBN: 978-1-68083-540-3\\
\\
\noindent \textit{HELM: The Holomorphic Embedding Load-Flow Method. Foundations and Implementations}\\
Antonio Trias\\
ISBN: 978-1-68083-516-8\\
\\
\noindent \textit{Combinatorial Optimization of Alternating Current Electric Power Systems}\\
Sid Chi-Kin Chau\\
ISBN: 978-1-68083-514-4

==> journaldata/ENT-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\begin{multicols}{1}
\journalchiefeditor{Albert N. Link}{University of North Carolina at Greensboro\\United States}
\journalchiefeditor{David B. Audretsch}{Indiana University\\United States}\\
\end{multicols}

\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Howard Aldrich}{University of North Carolina}
\journaleditor{Sharon Alvarez}{University of Denver}
\journaleditor{Per Davidsson}{Queensland University of Technology}
\journaleditor{Michael Frese}{National University of Singapore}
\journaleditor{William B. Gartner}{Copenhagen Business School}
\journaleditor{Magnus Henrekson}{IFN Stockholm}
\journaleditor{Michael A. Hitt}{Texas A\&M University}
\journaleditor{Joshua Lerner}{Harvard University}
\columnbreak
\journaleditor{Jeff McMullen}{Indiana University}
\journaleditor{P.R. Kumar}{Texas A\&M University}
\journaleditor{Maria Minniti}{Syracuse University}
\journaleditor{Simon Parker}{University of Western Ontario}
\journaleditor{Holger Patzelt}{TU Munich}
\journaleditor{Saras Sarasvathy}{University of Virginia}
\journaleditor{Roy Thurik}{Erasmus University}
\end{multicols*}
\end{editorialboard} 

==> journaldata/ENT-journaldata.tex <==
\definecolor{cerulean}{rgb}{0.0, 0.48, 0.65}
\colorlet{ENTcolor}{Cerulean}   %new color names can be defined before use
\journalcolor      {ENTcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Entrepreneurship}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ENT}
\journalurl        {http://www.nowpublishers.com/ENT}
\journalissnprint  {1551-3114}
\journalissnonline {1551-3122}
\journaldoi        {10.1561/03}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Entrepreneurship publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Nascent and start-up entrepreneurs}
\item{Opportunity recognition}
\item{New venture creation process}
\item{Business formation}
\item{Firm ownership}
\item{Market value and firm growth}
\item{Franchising}
\item{Managerial characteristics and behavior of entrepreneurs}
\item{Strategic alliances and networks}
\item{Government programs and public policy}
\item{Gender and ethnicity}
\columnbreak
\item{New business financing:}
	\begin{itemize}
\item{Business angels}
\item{Bank financing, debt, and trade credit}
\item{Venture capital and private equity capital}
\item{Public equity and IPOs} 
\end{itemize}
\item{Family-owned firms}
\item{Management structure, governance and performance}
\item{Corporate entrepreneurship}
\item{High technology:}
	\begin{itemize}
        \item{Technology-based new firms}
        \item{High-tech clusters}
        \end{itemize}
\item{Small business and economic growth}
\end{itemize}
 \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Entrepreneurship, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ENT-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Minority Entrepreneurship 2.0}\\
Timothy Bates\\
ISBN: 978-1-63828-048-4\\
\\
\noindent \textit{From the Metaphor to the Concept of the Entrepreneurial Journey in Entrepreneurship Research}\\
Tõnis Mets\\
ISBN: 978-1-63828-016-3\\
\\
\noindent \textit{Student Entrepreneurship: Reflections and Future Avenues for Research}\\
Bart Clarysse, Philippe Mustar and Lisa Dedeyne\\
ISBN: 978-1-63828-012-5\\
\\
\noindent \textit{Lumps, Bumps and Jumps in the Firm Growth Process}\\
Alex Coad\\
ISBN: 978-1-68083-960-9\\
\\
\noindent \textit{Understanding Entrepreneurial Failure: Conceptualizing Failure, Taking Stock, and Broadening the Scope of Failure Research}\\
Anna Jenkins\\
ISBN: 978-1-68083-950-0\\
\\
\noindent \textit{Pioneering Entrepreneurship Research: How, by Whom, and When}\\
Pontus Braunerhjelm, Martin Andersson and Johan Eklund\\
ISBN: 978-1-68083-948-7\\
\\




==> journaldata/FIN-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\begin{multicols}{1}
\journalchiefeditor{Sheridan Titman}{University of Texas at Austin\\United States}
\end{multicols}

\subsection{Associate Editors}
\begin{multicols}{1}
\journaleditor{Josef Zechner}{WU Vienna University of Economics and Finance}
\journaleditor{Chester Spatt}{Carnegie Mellon University}
\end{multicols}
\end{editorialboard} 

==> journaldata/FIN-journaldata.tex <==
\definecolor{ceruleanblue}{rgb}{0.16, 0.32, 0.75}
\colorlet{FINcolor}{ceruleanblue}   %new color names can be defined before use
\journalcolor      {FINcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Finance}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {FIN}
\journalurl        {http://www.nowpublishers.com/FIN}
\journalissnprint  {1567-2395}
\journalissnonline {1567-2409}
\journaldoi        {10.1561/05}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Finance publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Corporate Finance}
\begin{itemize}
\item{Corporate Governance}
\item{Corporate Financing}
\item{Dividend Policy and Capital Structure}
\item{Corporate Control}
\item{Investment Policy}
\item{Agency Theory and Information}
\end{itemize}
\end{itemize}
\columnbreak
\begin{itemize}
\item{Financial Markets}
\begin{itemize}
\item{Market Microstructure}
\item{Portfolio Theory}
\item{Financial Intermediation}
\item{Investment Banking}
\item{Market Efficiency}
\item{Security Issuance}
\item{Anomalies and Behavioral Finance}
\end{itemize}
\end{itemize}
\end{multicols}
%}
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
%\columnbreak
%\begin{itemize}
\item{Asset Pricing}
\begin{itemize}
\item{Asset-Pricing Theory}
\item{Asset-Pricing Models}
\item{Tax Effects}
\item{Liquidity} 
\item{Equity Risk Premium} 
\item{Pricing Models and Volatility} 
\item{Fixed Income Securities} 
\end{itemize}
\end{itemize}
\columnbreak
\begin{itemize}
\item{Derivatives}
\begin{itemize}
\item{Computational Finance}
\item{Futures Markets and Hedging}
\item{Financial Engineering}
\item{Interest Rate Derivatives}
\item{Credit Derivatives}
\item{Financial Econometrics}
\item{Estimating Volatilities and Correlations}
\end{itemize}
\end{itemize}
\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Finance, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/FIN-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Institutional Investors and Corporate Governance}\\
Amil Dasgupta, Vyacheslav Fos and Zacharias Sautner\\
ISBN: 978-1-68083-878-7\\
\\
\noindent \textit{The Implications of Heterogeneity and Inequality for Asset Pricing}\\
Stavros Panageas\\
ISBN: 978-1-68083-750-6\\
\\
\noindent \textit{Risk Sharing Within the Firm: A Primer}\\
Marco Pagano\\
ISBN: 978-1-68083-740-7\\
\\
\noindent \textit{The Economics of Credit Rating Agencies}\\
Francesco Sangiorgi and Chester Spatt\\
ISBN: 978-1-68083-380-5\\
\\
\noindent \textit{Initial Public Offerings: A Synthesis of the Literature and Directions for Future Research}\\
Michelle Lowry, Roni Michaely and Ekaterina Volkova\\
ISBN: 978-1-68083-340-9\\
\\
\noindent \textit{Privatization, State Capitalism, and State Ownership of Business in the 21st Century}\\
William L. Megginson\\
ISBN: 978-1-68083-338-6\\

==> journaldata/HCI-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Youn-Kyung Lim}{Korea Advanced Institute of Science and Technology}


\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Ben Bederson}{University of Maryland}
\journaleditor{Madeline Balaam}{KTH Royal Institute of Technology}
\journaleditor{Eun Kyoung Choe}{University of Maryland, College Park}
\journaleditor{Andy Cockburn}{University of Canterbury}
\journaleditor{Karrie Karahalios}{University of Illinois at Urbana-Champaign}
\journaleditor{Rohit Ashok Khot}{HAFP Research Lab, RMIT University}
\journaleditor{Uichin Lee}{Korea Advanced Institute of Science and Technology}
\journaleditor{Florian Mueller}{Exertion Games Lab, RMIT University}
\journaleditor{Bilge Mutlu}{University of Wisconsin-Madison}
\journaleditor{Marianna Obrist}{University of Sussex}
\journaleditor{Nuria Oliver}{Telefonica}
\journaleditor{Sameer Patil}{University of Utah}
\journaleditor{Orit Shaer}{Wellesley College}
\journaleditor{Desney S. Tan}{Microsoft Research}
\journaleditor{Koji Yatani}{University of Tokyo}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/HCI-journaldata.tex <==
\definecolor{pinegreen}{rgb}{0.0, 0.47, 0.44}
\colorlet{HCIcolor}{pinegreen}   %new color names can be defined before use
\journalcolor      {HCIcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Human-Computer Interaction}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {HCI}
\journalurl        {http://www.nowpublishers.com/HCI}
\journalissnprint  {1551-3955}
\journalissnonline {1551-3963}
\journaldoi        {10.1561/11}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Human-Computer Interaction publishes
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{History of the research community}
\item{Theory}
\item{Technology}
\item{Computer Supported Cooperative Work}
\item{Interdisciplinary influence}
\item{Advanced topics and trends}
\end{itemize}
%\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Human-Computer Interaction, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/HCI-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Modes of Uncertainty in HCI}\\
Robert Soden, Laura Devendorf, Richmond Wong, Yoko Akama and Ann Light\\
ISBN: 978-1-63828-054-5\\
\\
\noindent \textit{A Design Space of Sports Interaction Technology}\\
Dees B.W. Postma, Robby W. van Delden, Jeroen H. Koekoek, Wytse W. Walinga, Ivo M. van Hilvoorde, Bert Jan F. van Beijnum, Fahim A. Salim and Dennis Reidsma\\
ISBN: 978-1-63828-064-4\\
\\
\noindent \textit{Designs on Transcendence: Sketches of a TX machine}\\
Mark Blythe and Elizabeth Buie\\
ISBN: 978-1-68083-846-6\\
\\
\noindent \textit{Auditing Algorithms: Understanding Algorithmic Systems from the Outside In}\\
Danaë Metaxa, Joon Sung Park, Ronald E. Robertson, Karrie Karahalios, Christo Wilson, Jeff Hancock and Christian Sandvig\\
ISBN: 978-1-68083-916-6\\
\\
\noindent \textit{Design Framework for Interactive Highlighting Techniques}\\
Joshua Leung and Andy Cockburn\\
ISBN: 978-1-68083-924-1\\




==> journaldata/ICS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

%\begin{multicols*}{2}\raggedcolumns
\journalchiefeditor{Georges Gielen}{KU Leuven, Belgium}
%\end{multicols*}

\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Alison Burdett}{Sensium Healthcare, UK}
\journaleditor{Malgorzata Chrzanowska-Jeske}{Portland State University, USA}
\journaleditor{Paulo Diniz}{UFRJ, Brazil}
\journaleditor{Peter Kennedy}{University College Dublin, Ireland}
\journaleditor{Maciej Ogorzalek}{Jagiellonian University, Poland}
\journaleditor{Jan van der Spiegel}{University of Pennsylvania, USA}
\journaleditor{Ljiljana Trajkovic}{Simon Fraser University, USA}
%\end{multicols*}

\end{editorialboard} 

==> journaldata/ICS-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{ICScolor}{brickred}   %new color names can be defined before use
\journalcolor      {ICScolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Integrated Circuits and Systems}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ICS}
\journalurl        {http://www.nowpublishers.com/ICS}
\journalissnprint  {2693-9347}
\journalissnonline {2693-9355}
\journaldoi        {10.1561/35}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
 Integrated Circuits and Systems
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Analog, digital and mixed-signal circuits and systems}
\item{RF and mm-wave integrated circuits and systems}
\item{Wireless and wireline communication circuits and systems}
\item{Data converters and frequency generation}
\item{Power electronics and power management circuits}
\item{Biomedical circuits and systems}
\item{Sensor and imager circuits and cyber physical systems}
\item{Security and resilient circuits and systems}
\item{Circuits and systems in emerging non-CMOS technologies}
\item{Circuit theory, modeling, analysis and design methods}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Integrated Circuits and Systems, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ICS-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Emerging Trends of Biomedical Circuits and Systems}\\
Mohamad Sawan, Jie Yang, Mahdi Tarkhan, Jinbo Chen, Minqing Wang, Chuanqing Wang, Fen Xia and Yun-Hsuan Chen\\
ISBN: 978-1-68083-906-7\\
\\
\noindent \textit{Revisiting the Frontiers of Analog and Mixed-Signal Integrated Circuits Architectures and Techniques towards the future Internet of Everything (IoE) Applications}\\
Rui P. Martins, Pui-In Mak, Sai-Weng Sin, Man-Kay Law, Yan Zhu, Yan Lu, Jun Yin, Chi-Hang Chan, Yong Chen, Ka-Fai Un, Mo Huang, Minglei Zhang, Yang Jiang and Wei-Han Yu\\
ISBN: 978-1-68083-892-3\\
\\
\noindent \textit{Welcome to the World of Single-Slope Column-Level Analog-to-Digital Converters for CMOS Image Sensors}\\
Albert Theuwissen and Guy Meynants\\
ISBN: 978-1-68083-812-1\\
\\




==> journaldata/INR-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Yiqun Liu}{Tsinghua University\\China}
\journalchiefeditor{Diane Kelly}{University of Tennessee\\USA}



\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Barbara Poblete}{University of Chile}
\journaleditor{Chirag Shah}{University of Washington}
\journaleditor{Claudia Hauff}{Delft University of Technology}
\journaleditor{Dawei Yin}{Baidu inc.}
\journaleditor{Ellen M. Voorhees}{National Institute of Standards and Technology}
\journaleditor{Hang Li}{Bytedance Technology}
\journaleditor{Isabelle Moulinier}{Independent}
\journaleditor{Jaap Kamps}{University of Amsterdam}
\journaleditor{Lorraine Goeuriot}{Université Grenoble Alpes}
\columnbreak
\journaleditor{Lynda Tamine}{University of Toulouse}
\journaleditor{Maarten de Rijke}{University of Amsterdam and Ahold Delhaize}
\journaleditor{Mandar Mitra}{Indian Statistical Institute}
\journaleditor{Rodrygo Luis Teodoro Santos}{Universidade Federal de Minas Gerais}
\journaleditor{Ruihua Song}{Renmin University of China}
\journaleditor{Shane Culpepper}{RMIT}
\journaleditor{Xiangnan He}{University of Science and Technology of China}
\journaleditor{Xuanjing Huang}{Fudan University}
\journaleditor{Yubin Kim}{Etsy}
\journaleditor{Zi Helen Huang}{University of Queensland}
\end{multicols*}
\end{editorialboard} 

==> journaldata/INR-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{INRcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {INRcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Information Retrieval}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {INR}
\journalurl        {http://www.nowpublishers.com/INR}
\journalissnprint  {1554-0669}
\journalissnonline {1554-0677}
\journaldoi        {10.1561/15}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Information Retrieval publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Applications of IR}
\item{Architectures for IR}
\item{Collaborative filtering and recommender systems}
\item{Cross-lingual and multilingual IR}
\item{Distributed IR and federated search}
\item{Evaluation issues and test collections for IR}
\item{Formal models and language models for IR}
\item{IR on mobile platforms}
\item{Indexing and retrieval of structured documents}
\item{Information categorization and clustering}
\item{Information extraction}
\item{Information filtering and routing}
\item{Metasearch, rank aggregation and data fusion}
\item{Natural language processing for IR}
\item{Performance issues for IR systems, including algorithms, data structures, optimization techniques, and scalability}
\item{Question answering}
\item{Summarization of single documents, multiple documents, and corpora}
\item{Text mining}
\item{Topic detection and tracking}
\item{Usability, interactivity, and visualization issues in IR}
\item{User modelling and user studies for IR}
\item{Web search}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Information Retrieval, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 5 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/INR-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Fairness in Information Access Systems}\\
Michael D. Ekstrand, Anubrata Das, Robin Burke and Fernando Diaz\\
ISBN: 978-1-63828-040-8\\

\noindent \textit{Deep Learning for Dialogue Systems: Chit-Chat and Beyond}\\
Rui Yan, Juntao Li and Zhou Yu\\
ISBN: 978-1-63828-022-4\\

\noindent \textit{Search Interface Design and Evaluation}\\
Chang Liu, Ying-Hsang Liu, Jingjing Liu and Ralf Bierig\\
ISBN: 978-1-68083-922-7\\

\noindent \textit{Psychology-informed Recommender Systems}\\
Elisabeth Lex, Dominik Kowald, Paul Seitlinger, Thi Ngoc Trang Tran, Alexander Felfernig and Markus Schedl\\
ISBN: 978-1-68083-844-2\\

\noindent \textit{Search and Discovery in Personal Email Collections}\\
Michael Bendersky, Xuanhui Wang, Marc Najork and Donald Metzler\\
ISBN: 978-1-68083-838-1\\






==> journaldata/ISY-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

%\begin{multicols}{1}
\journalchiefeditor{David Paradice}{Auburn University\\United States}
%\end{multicols}

\subsection{Honorary Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Alan R. Dennis}{Kelley School of Business, Indiana University}
\journaleditor{Joey George}{Iowa State University}
%\end{multicols*}

\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Alan Hevner}{University of South Florida}
\journaleditor{K.D. Joshi}{University of Nevada - Reno, USA}
\journaleditor{Uday Kulkarni}{Arizona State University, USA}
\journaleditor{Michael Prietula}{Emory University, USA}
\journaleditor{Carol Saunders}{University of Central Florida}
\journaleditor{Veda Storey}{Georgia State University}
\journaleditor{Brad Wheeler}{Indiana University, USA}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/ISY-journaldata.tex <==
\definecolor{regalia}{rgb}{0.32, 0.18, 0.5}
\colorlet{ISYcolor}{regalia}   %new color names can be defined before use
\journalcolor      {ISYcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Information Systems}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ISY}
\journalurl        {http://www.nowpublishers.com/ISY}
\journalissnprint  {2331-1231}
\journalissnonline {2331-124X}
\journaldoi        {10.1561/29}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Information Systems publishes
 survey and tutorial articles in the following topics: 
%\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{IS and Individuals}
\item{IS and Groups}
\item{IS and Organizations}
\item{IS and Industries}
\item{IS and Society}
\item{IS Development}
\item{IS Economics}
\item{IS Management}
\item{IS Research Methods}
\end{itemize}
% \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Information Systems, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ISY-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Information Technology Alignment and Innovation: 30 Years of Intersecting Research}\\
Yolande E. Chan, Rashmi Krishnamurthy and Ali S. Ghawe\\
ISBN: 978-1-68083-816-9\\
\\
\noindent \textit{Process Theory: Background, Opportunity, and Challenges}\\
Fred Niederman\\
ISBN: 978-1-68083-806-0\\
\\
\noindent \textit{IT Project Management: Lessons Learned from Project Retrospectives 1999–2020}\\
R. Ryan Nelson\\
ISBN: 978-1-68083-776-6\\
\\
\noindent \textit{Speech Analytics for Actionable Insights: Current Status, Recommendation, and Guidance}\\
J. P. Shim, Aaron M. French and Bikesh Upreti\\
ISBN: 978-1-68083-696-7\\
\\
\noindent \textit{A Review of Personality in Human–Robot Interactions}\\
Lionel P. Robert Jr., Rasha Alahmad, Connor Esterwood, Sangmi Kim, Sangseok You and Qiaoning Zhang\\
ISBN: 978-1-68083-662-2\\



==> journaldata/MAL-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Michael Jordan}{University of California, Berkeley\\United States}



\subsection{Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Peter Bartlett}{UC Berkeley}
\journaleditor{Yoshua Bengio}{Universit{\'e} de Montr{\'e}al}
\journaleditor{Avrim Blum}{Toyota Technological Institute}
\journaleditor{Craig Boutilier}{University of Toronto}
\journaleditor{Stephen Boyd}{Stanford University}
\journaleditor{Carla Brodley}{Northeastern University}
\journaleditor{Inderjit Dhillon}{Texas at Austin}
\journaleditor{Jerome Friedman}{Stanford University}
\journaleditor{Kenji Fukumizu}{ISM}
\journaleditor{Zoubin Ghahramani}{Cambridge University}
\journaleditor{David Heckerman}{Amazon}
\journaleditor{Tom Heskes}{Radboud University}
\journaleditor{Geoffrey Hinton}{University of Toronto}
\journaleditor{Aapo Hyvarinen}{Helsinki IIT}
\journaleditor{Leslie Pack Kaelbling}{MIT}
\journaleditor{Michael Kearns}{UPenn}
\journaleditor{Daphne Koller}{Stanford University}
\journaleditor{John Lafferty}{Yale}
\journaleditor{Michael Littman}{Brown University}
\journaleditor{Gabor Lugosi}{Pompeu Fabra}
\journaleditor{David Madigan}{Columbia University}
\journaleditor{Pascal Massart}{Universit{\'e} de Paris-Sud}
\journaleditor{Andrew McCallum}{University of Massachusetts Amherst}
\journaleditor{Marina Meila}{University of Washington}
\journaleditor{Andrew Moore}{CMU}
\journaleditor{John Platt}{Microsoft Research}
\journaleditor{Luc de Raedt}{KU Leuven}
\journaleditor{Christian Robert}{Paris-Dauphine}
\journaleditor{Sunita Sarawagi}{IIT Bombay}
\journaleditor{Robert Schapire}{Microsoft Research}
\journaleditor{Bernhard Schoelkopf}{Max Planck Institute}
\journaleditor{Richard Sutton}{University of Alberta}
\journaleditor{Larry Wasserman}{CMU}
\journaleditor{Bin Yu}{UC Berkeley}
\end{multicols*}
\end{editorialboard} 

==> journaldata/MAL-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{MALcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {MALcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Machine Learning}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MAL}
\journalurl        {http://www.nowpublishers.com/MAL}
\journalissnprint  {1935-8237}
\journalissnonline {1935-8245}
\journaldoi        {10.1561/22}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Machine Learning publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Adaptive control and signal processing}
\item{Applications and case studies}
\item{Behavioral, cognitive and neural learning}
\item{Bayesian learning}
\item{Classification and prediction}
\item{Clustering}
\item{Data mining}
\item{Dimensionality reduction}
\item{Evaluation}
\item{Game theoretic learning}
\item{Graphical models}
\item{Independent component analysis}
\item{Inductive logic programming}
\item{Kernel methods}
\item{Markov chain Monte Carlo}
\item{Model choice}
\item{Nonparametric methods}
\item{Online learning}
\item{Optimization}
\item{Reinforcement learning}
\item{Relational learning}
\item{Robustness}
\item{Spectral methods}
\item{Statistical learning theory}
\item{Variational inference}
\item{Visualization}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Machine Learning, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 6 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/MAL-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Learning in Repeated Auctions}\\
Thomas Nedelec, Clément Calauzènes, Noureddine El Karoui and Vianney Perchet\\
ISBN: 978-1-68083-938-8\\
\\
\noindent \textit{Dynamical Variational Autoencoders: A Comprehensive Review}\\
Laurent Girin, Simon Leglaive, Xiaoyu Bie, Julien Diard, Thomas Hueber and Xavier Alameda-Pineda\\
ISBN: 978-1-68083-912-8\\
\\
\noindent \textit{Machine Learning for Automated Theorem Proving: Learning to Solve SAT and QSATe}\\
Sean B. Holden\\
ISBN: 978-1-68083-898-5\\
\\
\noindent \textit{Spectral Methods for Data Science: A Statistical Perspective}\\
Yuxin Chen, Yuejie Chi, Jianqing Fan and Cong Ma\\
ISBN: 978-1-68083-896-1\\
\\
\noindent \textit{Tensor Regression}\\
Jiani Liu, Ce Zhu, Zhen Long and Yipeng Liu\\
ISBN: 978-1-68083-886-2\\
\\
\noindent \textit{Minimum-Distortion Embedding}\\
Akshay Agrawal, Alnur Ali and Stephen Boyd\\
ISBN: 978-1-68083-888-6\\
\\

==> journaldata/MGT-editorialboard.tex <==
%ACG-Editorialboard.

\begin{editorialboard}

\subsection{Editors-in-Chief}

\begin{multicols}{2}\raggedright
\journalchiefeditor{Nicholas S. Argyres}{Olin Business School, Washington University\\United States}
\journalchiefeditor{Timothy M. Devinney}{Leeds University Business School\\United Kingdom}
\journalchiefeditor{James Campbell Quick}{The University of Texas at Arlington\\United States}
\end{multicols}

\subsection{Editors}
\begin{multicols}{3}\raggedright \raggedcolumns
\renewcommand\journaleditor[2]{\par\textbf{#1}\\#2}%
\subsubsection{\footnotesize International Business}

\journaleditor{Gabriel R.G. Benito}{BI Norwegian School of Management}
\journaleditor{Allan Bird}{Northeastern University}
\journaleditor{Julian Birkinshaw}{London Business School}
\journaleditor{Peter Buckley}{University of Leeds}
\journaleditor{Saul Estrin}{London School of Economics}
\journaleditor{Sarianna Lundin}{University of Bremen}
\journaleditor{Xavier Martin}{Tilburg University} 
\journaleditor{Ram Mudambi}{Temple University}

\columnbreak

\subsubsection{\footnotesize Organizational Behavior}

\journaleditor{Myrtle Bell}{University of Texas at Arlington}
\journaleditor{Cary Cooper}{Lancaster University}
\journaleditor{Richard Griffin}{Texas A\&M University}
\journaleditor{Sean Hannah}{Wake Forest University}
\journaleditor{Debra Nelson}{Oklahoma State University}
\journaleditor{Pamela Perrewe}{Florida State University}

\columnbreak

\subsubsection{\footnotesize Strategy}

\journaleditor{Rajshree Agarwal}{University of Maryland}
\journaleditor{Marvin Lieberman}{UCLA}) 
\journaleditor{Michael Lenox}{University of Virginia}
\journaleditor{Joseph Mahoney}{University of Illinois at Urbana-Champaign}
\journaleditor{Jesper Sørensen}{Stanford University}
\journaleditor{Olav Sorenson}{Yale University}
\end{multicols}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/MGT-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{MGTcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {MGTcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Management}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MGT}
\journalurl        {http://www.nowpublishers.com/MGT}
\journalissnprint  {2475-6946}
\journalissnonline {2475-6954}
\journaldoi        {10.1561/34}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Management publishes
 survey and tutorial articles in the following topics:
% \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{International Business}
\item{Organizational Behavior}
\item{Strategic Management}
\end{itemize}
 %\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Management, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/MIC-editorialboard.tex <==
%MIC-Editorialboard.

\begin{editorialboard}

%\subsection{Editor-in-Chief}

\journalchiefeditor{W. Kip Viscusi}{Vanderbilt University Law School\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Richard Carson}{University of California, San Diego}
\journaleditor{William Gentry}{Williams College}
\journaleditor{Tom Kniesner}{Syracuse University}
\journaleditor{Mark V. Pauly}{University of Pennsylvania}
\journaleditor{Yossi Spiegel}{Tel Aviv University}
\journaleditor{William Zame}{University of California, Los Angeles}
\journaleditor{James Ziliak}{University of Kentucky}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/MIC-journaldata.tex <==
\definecolor{pinegreen}{rgb}{0.0, 0.47, 0.44}
\colorlet{MICcolor}{pinegreen}   %new color names can be defined before use   %new color names can be defined before use
\journalcolor      {MICcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Microeconomics}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MIC}
\journalurl        {http://www.nowpublishers.com/MIC}
\journalissnprint  {1547-9846}
\journalissnonline {1547-9854}
\journaldoi        {10.1561/07}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Microeconomics publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Environmental economics}
\item{Health economics}
\item{Industrial organization}
\item{Labor economics}
\item{Law and economics}
\item{Public economics}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Microeconomics, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/MIC-seriespage.tex <==
\vspace{12pt}
\vspace{12pt}
\noindent \textit{Behavioral Economics of Multiperiod Insurance Purchasing Behavior: The Role of Emotions}\\
Howard Kunreuther and Mark Pauly
\\ISBN: 978-1-68083-524-3
\\
\\
\noindent \textit{Trade and Climate Change: Focus on Carbon Leakage, Border Carbon Adjustments and WTO Consistency}\\
ZhongXiang Zhang
\\ISBN: 978-1-68083-482-6
\\
\\
\noindent \textit{Natural Gas Pipeline Regulation in the United States: Past, Present, and Future}\\
Matthew E. Oliver
\\ISBN: 978-1-68083-452-9
\\
\\
\noindent \textit{The U.S. Market for Uranium: 70 Years of History}\\
Charles F. Mason
\\ISBN: 978-1-68083-382-9
\\
\\
\noindent \textit{Game Theory and Water Resources: Critical Review of its Contributions, Progress and Remaining Challenges}\\
Ariel Dinar and Margaret Hogarth
\\ISBN: 978-1-68083-016-3


==> journaldata/MKT-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Jehoshua Eliashberg}{University of Pennsylvania}

\subsection{Associate Editor}

\journaleditor{Bernd Schmitt}{Columbia University}


\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Dawn Iacobucci}{Vanderbilt University}
\journaleditor{Ganesh Iyeri}{University of California, Berkeley}
\journaleditor{Anirban Mukhopadhyayi}{HKUST}
\journaleditor{Sharon Ngi}{Nanyang Technological University}
\journaleditor{Gerrit van Bruggeni}{Erasmus University}
\journaleditor{Miguel Villas Boasi}{University of California, Berkeley}
\journaleditor{Hema Yoganarasimhani}{University of Washington}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/MKT-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{MKTcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {MKTcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Marketing}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MKT}
\journalurl        {http://www.nowpublishers.com/MKT}
\journalissnprint  {1555-0753}
\journalissnonline {1555-0761}
\journaldoi        {10.1561/17}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Marketing publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{B2B Marketing}
\item{Bayesian Models}
\item{Behavioral Decision Making}
\item{Branding and Brand Equity}
\item{Channel Management}
\item{Choice Modeling}
\item{Comparative Market Structure}
\item{Competitive Marketing Strategy}
\item{Conjoint Analysis}
\item{Customer Equity}
\item{Customer Relationship Management}
\item{Game Theoretic Models}
\item{Group Choice and Negotiation}
\item{Discrete Choice Models}
\item{Individual Decision Making}
\item{Marketing Decisions Models}
\item{Market Forecasting}
\item{Marketing Information Systems}
\item{Market Response Models}
\item{Market Segmentation}
\item{Market Share Analysis}
\item{Multi-channel Marketing}
\item{New Product Diffusion}
\item{Pricing Models}
\item{Product Development}
\item{Product Innovation}
\item{Sales Forecasting}
\item{Sales Force Management}
\item{Sales Promotion}
\item{Services Marketing}
\item{Stochastic Model}
\end{itemize}
 \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Marketing, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/MKT-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Language Research in Marketing}\\
Ann Kronrod\\
ISBN: 978-1-68083-966-1\\
\\
\noindent \textit{Reflections of Eminent Marketing Scholars}\\
Dawn Iacobucci\\
ISBN: 978-1-68083-954-8\\
\\
\noindent \textit{Social Media Analytics and Its Applications in Marketing}\\
Sangkil Moon and Dawn Iacobucci\\
ISBN: 978-1-68083-952-4\\
\\
\noindent \textit{Privacy and Consumer Empowerment in Online Advertising}\\
W. Jason Choi and Kinshuk Jerath\\
ISBN: 978-1-68083-920-3\\
\\
\noindent \textit{Studying Healthcare from a Marketing Perspective}\\
Dawn Iacobucci and Deidre Popovich\\
ISBN: 978-1-68083-918-0\\
\\
\noindent \textit{Aggregate Advertising Expenditure in the U.S. Economy: Measurement and Growth Issues in the Digital Era}\\
Alvin J. Silk and Ernst R. Berndt\\
ISBN: 978-1-68083-872-5\\
\\



==> journaldata/NET-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Anthony Ephremides}{University of Maryland\\United States}



\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Fran\c{c}ois Baccelli}{University of Texas, Austin}
\journaleditor{Victor Bahl}{Microsoft Research}
\journaleditor{Helmut B\"{o}lcskei}{ETH Zurich}
\journaleditor{J.J. Garcia-Luna Aceves}{UC Santa Cruz}
\journaleditor{Andrea Goldsmith}{Stanford University}
\journaleditor{Roch Guerin}{Washington University in Saint Louis}
\journaleditor{Bruce Hajek}{UIUC}
\journaleditor{Jean-Pierre Hubaux}{EPFL}
\journaleditor{Frank Kelly}{University of Cambridge}
\journaleditor{P.R. Kumar}{Texas A\&M University}
\journaleditor{Steven Low}{Caltech}
\journaleditor{Eytan Modiano}{MIT}
\columnbreak
\journaleditor{Keith Ross}{Polytechnic Institute of NYU}
\journaleditor{Henning Schulzrinne}{Columbia University}
\journaleditor{Mani Srivastava}{UCLA}
\journaleditor{Leandros Tassiulas}{Yale University}
\journaleditor{Lang Tong}{Cornell University}
\journaleditor{Ozan Tonguz}{Carnegie Mellon University}
\journaleditor{Don Towsley}{University of Massachusetts, Amherst}
\journaleditor{Nitin Vaidya}{UIUC}
\journaleditor{Pravin Varaiya}{UC Berkeley}
\journaleditor{Roy Yates}{Rutgers University}
\journaleditor{Raymond Yeung}{Chinese University of Hong Kong}
\end{multicols*}
\end{editorialboard} 

==> journaldata/NET-journaldata.tex <==
\definecolor{cerise}{rgb}{0.87, 0.19, 0.39}
\colorlet{NETcolor}{cerise}   %new color names can be defined before use
\journalcolor      {NETcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Networking}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {NET}
\journalurl        {http://www.nowpublishers.com/NET}
\journalissnprint  {1554-057X}
\journalissnonline {1554-0588}
\journaldoi        {10.1561/13}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Networking publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Modeling and Analysis of:}
	\begin{itemize}
	\item{Ad Hoc Wireless Networks}
	\item{Sensor Networks}
	\item{Optical Networks}
	\item{Local Area Networks}
	\item{Satellite and Hybrid Networks}
	\item{Cellular Networks}
	\item{Internet and Web Services}
	\end{itemize}
\item{Protocols and Cross-Layer Design}
\item{Network Coding}
\item{Energy-Efficiency Incentives/Pricing/Utility-based}
\item{Games (co-operative or not)}
\item{Security}
\item{Scalability}
\item{Topology}
\item{Control/Graph-theoretic models}
\item{Dynamics and Asymptotic Behavior of Networks}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Networking, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/NET-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Age of Information: A New Concept, Metric, and Tool}\\
Antzela Kosta, Nikolaos Pappas and Vangelis Angelakis\\
ISBN: 978-1-68083-360-7\\
\\
\noindent \textit{Network and Protocol Architectures for Future Satellite Systems}\\
Tomaso de Cola, Alberto Ginesi, Giovanni Giambene,\\ George C. Polyzos, Vasilios A. Siris, Nikos Fotiou and Yiannis Thomas\\
ISBN: 978-1-68083-334-8\\
\\
\noindent \textit{Duality of the Max-Plus and Min-Plus Network Calculus}\\
Jorg Liebeherr\\
ISBN: 978-1-68083-294-5\\
\\
\noindent \textit{Opportunistic Routing in Wireless Networks}\\
Tara Javidi and Eric Van Buhler\\
ISBN: 978-1-68083-150-4

==> journaldata/NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> journaldata/OPT-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

%\begin{multicols}{1}
\journalchiefeditor{Garud Iyengar}{Columbia University, USA}
%\end{multicols}

\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Dimitris Bertsimas}{Massachusetts Institute of Technology}
\journaleditor{John R. Birge}{The University of Chicago}
\journaleditor{Robert E. Bixby}{Rice University}
\journaleditor{Emmanuel Candes}{Stanford University}
\journaleditor{David Donoho}{Stanford University}
\journaleditor{Laurent El Ghaoui}{University of California, Berkeley}
\journaleditor{Donald Goldfarb}{Columbia University}
\journaleditor{Michael I. Jordan}{University of California, Berkeley}
\journaleditor{Zhi-Quan (Tom) Luo}{University of Minnesota, Twin Cites}
\journaleditor{George L. Nemhauser}{Georgia Institute of Technology}
\journaleditor{Arkadi Nemirovski}{Georgia Institute of Technology}
\columnbreak
\journaleditor{Yurii Nesterov}{HSE University}
\journaleditor{Jorge Nocedal}{Northwestern University}
\journaleditor{Pablo A. Parrilo}{Massachusetts Institute of Technology}
\journaleditor{Boris T. Polyak}{Institute for Control Science, Moscow}
\journaleditor{Tam\'as Terlaky}{Lehigh University}
\journaleditor{Michael J. Todd}{Cornell University}
\journaleditor{Kim-Chuan Toh}{National University of Singapore}
\journaleditor{John N. Tsitsiklis}{Massachusetts Institute of Technology}
\journaleditor{Lieven Vandenberghe}{University of California, Los Angeles}
\journaleditor{Robert J. Vanderbei}{Princeton University}
\journaleditor{Stephen J. Wright}{University of Wisconsin}
\end{multicols*}
\end{editorialboard} 

==> journaldata/OPT-journaldata.tex <==
\definecolor{cerulean}{rgb}{0.0, 0.48, 0.65}
\colorlet{OPTcolor}{Cerulean}   %new color names can be defined before use
\journalcolor      {OPTcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Optimization}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {OPT}
\journalurl        {http://www.nowpublishers.com/OPT}
\journalissnprint  {2167-3888}
\journalissnonline {2167-3918}
\journaldoi        {10.1561/24}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Optimization publishes
 survey and tutorial articles in the following topics: 
%\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{algorithm design, analysis, and implementation (especially, on modern computing platforms}
\item{models and modeling systems, new optimization formulations for practical problems}
\item{applications of optimization in machine learning, statistics, and data analysis, signal and image processing, computational economics and finance, engineering design, scheduling and resource allocation, and other areas}
\end{itemize}
 %\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Optimization, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/OPT-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Algorithms for Verifying Deep Neural Networks}\\
Changliu Liu, Tomer Arnon, Christopher Lazarus, Christopher Strong, Clark Barrett and Mykel J. Kochenderfer\\
ISBN: 978-1-68083-786-5\\
\\
\noindent \textit{Distributionally Robust Learning}\\
Ruidi Chen and Ioannis Ch. Paschalidis\\
ISBN: 978-1-68083-772-8\\
\\
\noindent \textit{Atomic Decomposition via Polar Alignment: The Geometry of Structured Optimization}\\
Zhenan Fan, Halyun Jeong, Yifan Sun and Michael P. Friedlander\\
ISBN: 978-1-68083-742-1\\
\\
\noindent \textit{Optimization Methods for Financial Index Tracking: From Theory to Practice}\\
Konstantinos Benidis, Yiyong Feng and Daniel P. Palomar\\
ISBN: 978-1-68083-464-2\\
\\
\noindent \textit{The Many Faces of Degeneracy in Conic Optimization}\\
Dmitriy Drusvyatskiy and Henry Wolkowicz\\
ISBN: 978-1-68083-390-4\\

==> journaldata/PGL-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Rupak Majumdari}{Max Planck Institute for Software Systems}


\subsection{Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Mart\'in Abadi}{Google and UC Santa Cruz}
\journaleditor{Anindya Banerjee}{IMDEA Software Instituet}
\journaleditor{Patrick Cousot}{ENS, Paris and NYU}
\journaleditor{Oege De Moor}{University of Oxford}
\journaleditor{Matthias Felleisen}{Northeastern University}
\journaleditor{John Field}{Google}
\journaleditor{Cormac Flanagan}{UC Santa Cruz}
\journaleditor{Philippa Gardner}{Imperial College}
\journaleditor{Andrew Gordon}{Microsoft Research and University of Edinburgh}
\journaleditor{Dan Grossman}{University of Washington}
\journaleditor{Robert Harper}{CMU}
\journaleditor{Tim Harris}{Amazon}
\journaleditor{Fritz Henglein}{University of Copenhagen}
\journaleditor{Rupak Majumdar}{MPI and UCLA}
\journaleditor{Kenneth McMillan}{Microsoft Research}
\journaleditor{J. Eliot B. Moss}{University of Massachusetts, Amherst}
\journaleditor{Andrew C. Myers}{Cornell University}
\journaleditor{Hanne Riis Nielson}{Technical University of Denmark}
\journaleditor{Peter O'Hearni}{University College London}
\journaleditor{Benjamin C. Pierce}{University of Pennsylvania}
\journaleditor{Andrew Pittsi}{University of Cambridge}
\journaleditor{Ganesan Ramalingami}{Microsoft Research}
\journaleditor{Mooly Sagiv}{Tel Aviv University}
\journaleditor{Davide Sangiorgi}{University of Bologna}
\journaleditor{David Schmidt}{Kansas State University}
\journaleditor{Peter Sewell}{University of Cambridge}
\journaleditor{Scott Stoller}{Stony Brook University}
\journaleditor{Peter Stuckey}{University of Melbourne}
\journaleditor{Jan Vitek}{Northeastern University}
\journaleditor{Philip Wadler}{University of Edinburgh}
\journaleditor{David Walker}{Princeton University}
\journaleditor{Stephanie Weirich}{University of Pennsylvania}
\end{multicols*}
\end{editorialboard} 

==> journaldata/PGL-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{PGLcolor}{brickred}   %new color names can be defined before use
\journalcolor      {PGLcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Programming Languages}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {PGL}
\journalurl        {http://www.nowpublishers.com/PGL}
\journalissnprint  {2325-1107}
\journalissnonline {2325-1131}
\journaldoi        {10.1561/25}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Programming Languages publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Abstract Interpretation}
\item{Compilation and Interpretation Techniques}
\item{Domain Specific Languages}
\item{Formal Semantics, including Lambda Calculi, Process Calculi, and Process Algebra}
\item{Language Paradigms}
    \item{Mechanical Proof Checking}
    \item{Memory Management}
    \item{Partial Evaluation}
    \item{Program Logic}
    \item{Programming Language Implementation}
    \item{Programming Language Security}
    \item{Programming Languages for Concurrency}
    \item{Programming Languages for Parallelism}
    \item{Program Synthesis}
    \item{Program Transformations and Optimizations}
    \item{Program Verification}
    \item{Runtime Techniques for Programming Languages}
    \item{Software Model Checking}
    \item{Static and Dynamic Program Analysis}
    \item{Type Theory and Type Systems}
\end{itemize}
\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
 Programming Languages, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/PGL-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Introduction to Neural Network Verification}\\
Aws Albarghouthi\\
ISBN: 978-1-68083-910-4\\
\\
\noindent \textit{Refinement Types: A Tutorial}\\
Ranjit Jhala and Niki Vazou\\
ISBN: 978-1-68083-884-8\\
\\
\noindent \textit{Shape Analysis}\\
Bor-Yuh Evan Chang, Cezara Drăgoi, Roman Manevich, Noam Rinetzky and Xavier Rival\\
ISBN: 978-1-68083-732-2\\
\\
\noindent \textit{Progress of Concurrent Objects}\\
Hongjin Liang and Xinyu Feng\\
ISBN: 978-1-68083-672-1\\
\\
\noindent \textit{QED at Large: A Survey of Engineering of Formally Verified \\Software}\\
Talia Ringer, Karl Palmskog, Ilya Sergey, Milos Gligoric and \\Zachary Tatlock\\
ISBN: 978-1-68083-594-6\\
\\
\noindent \textit{Reconciling Abstraction with High Performance: A MetaOCaml \\approach}\\
Oleg Kiselyov\\
ISBN: 978-1-68083-436-9

==> journaldata/ROB-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}
\journalchiefeditor{Julie Shah}{Massachusetts Institute of Technology}

\subsection{Honorary Editors}
\journaleditor{Henrik Christensen}{University of California, San Diego}
\journaleditor{Roland Siegwart}{ETH Zurich}


\subsection{Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Minoru Asada}{Osaka University}
\journaleditor{Antonio Bicchi}{University of Pisa}
\journaleditor{Aude Billard}{EPFL}
\journaleditor{Cynthia Breazeal}{Massachusetts Institute of Technology}
\journaleditor{Oliver Brock}{TU Berlin}
\journaleditor{Wolfram Burgard}{University of Freiburg}
\journaleditor{Udo Frese}{University of Bremen}
\journaleditor{Ken Goldberg}{University of California, Berkeley}
\journaleditor{Hiroshi Ishiguro}{Osaka University}
\journaleditor{Makoto Kaneko}{Osaka University}
\journaleditor{Danica Kragic}{KTH Stockholm}
\journaleditor{Vijay Kumar}{University of Pennsylvania}
\journaleditor{Simon Lacroix}{LAAS}
\journaleditor{Christian Laugier}{INRIA}
\journaleditor{Steve LaValle}{University of Illinois at Urbana-Champaign}
\journaleditor{Yoshihiko Nakamura}{The University of Tokyo}
\journaleditor{Brad Nelson}{ETH Zurich}
\journaleditor{Paul Newman}{University of Oxford}
\journaleditor{Daniela Rus}{Massachusetts Institute of Technology}
\journaleditor{Giulio Sandini}{University of Genova}
\journaleditor{Sebastian Thrun}{Stanford University}
\journaleditor{Manuela Veloso}{Carnegie Mellon University}
\journaleditor{Markus Vincze}{Vienna University}
\journaleditor{Alex Zelinsky}{DSTG}
\end{multicols*}
\end{editorialboard} 

==> journaldata/ROB-journaldata.tex <==
\definecolor{pinegreen}{rgb}{0.0, 0.47, 0.44}
\colorlet{ROBcolor}{pinegreen}   %new color names can be defined before use
\journalcolor      {ROBcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Robotics}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ROB}
\journalurl        {http://www.nowpublishers.com/ROB}
\journalissnprint  {1935-8253}
\journalissnonline {1935-8261}
\journaldoi        {10.1561/23}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Robotics publishes
 survey and tutorial articles in the following topics:
\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Mathematical modelling}
\item{Kinematics}
\item{Dynamics}
\item{Estimation Methods}
\item{Robot Control}
\item{Planning}
\item{Artificial Intelligence in Robotics}
\item{Software Systems and Architectures}
\item{Mechanisms and Actuators}
\item{Sensors and Estimation}
\item{Planning and Control}
\item{Human-Robot Interaction}
\item{Industrial Robotics}
\item{Service Robotics }
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Robotics, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ROB-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Adoption of Robots for Disasters: Lessons from the Response to COVID-19}\\
Robin R. Murphy, Vignesh B.M. Gandudi, Justin Adams, Angela Clendenin and Jason Moats\\
ISBN: 978-1-68083-862-6\\
\\
\noindent \textit{Cybersecurity in Robotics: Challenges, Quantitative Modeling, and Practice}\\
Quanyan Zhu, Stefan Rass, Bernhard Dieber and Víctor Mayoral Vilches\\
ISBN: 978-1-68083-860-2\\
\\
\noindent \textit{A Roadmap for US Robotics – From Internet to Robotics 2020 Edition}\\
Henrik Christensen, Nancy Amato, Holly Yanco, Maja Mataric, Howie Choset, Ann Drobnis, Ken Goldberg, Jessy Grizzle, Gregory Hager, John Hollerbach, Seth Hutchinson, Venkat Krovi, Daniel Lee, Bill Smart, Jeff Trinkle and Gaurav Sukhatme\\
ISBN: 978-1-68083-858-9\\
\\
\noindent \textit{The State of Industrial Robotics: Emerging Technologies, Challenges, and Key Research Directions}\\
Lindsay Sanneman, Christopher Fourie and Julie A. Shah\\
ISBN: 978-1-68083-800-8\\
\\
\noindent \textit{Semantics for Robotic Mapping, Perception and Interaction: A Survey}\\
Sourav Garg, Niko Sünderhauf, Feras Dayoub, Douglas Morrison, Akansel Cosgun, Gustavo Carneiro, Qi Wu, Tat-Jun Chin, Ian Reid, Stephen Gould, Peter Corke and Michael Milford\\
ISBN: 978-1-68083-768-1\\


==> journaldata/SEC-editorialboard.tex <==
%SEC-Editorialboard.

\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Anupam Datta}{Carnegie Mellon University, USA}
\journalchiefeditor{Jeannette Wing}{Columbia University, USA}


\subsection{Editors}
\begin{multicols}{2}\raggedcolumns
\journaleditor{Mart\'in Abadi}{Google and University of California, Santa Cruz}
\journaleditor{Michael Backes}{Saarland University}
\journaleditor{Dan Boneh}{Stanford University, USA}
\journaleditor{V\'eronique Cortier}{LORIA, CNRS, France}
\journaleditor{Lorrie Cranor}{Carnegie Mellon University}
\journaleditor{C\'edric Fournet}{Microsoft Research}
\journaleditor{Virgil Gligor}{Carnegie Mellon University}
\journaleditor{Jean-Pierre Hubaux}{EPFL}
\journaleditor{Deirdre Mulligan}{University of California, Berkeley}
\journaleditor{Andrew Myers}{Cornell University}
\journaleditor{Helen Nissenbaum}{New York University}
\journaleditor{Michael Reiter}{University of North Carolina}
\journaleditor{Shankar Sastry}{University of California, Berkeley}
\journaleditor{Dawn Song}{University of California, Berkeley}
\journaleditor{Daniel Weitzner}{Massachusetts Institute of Technology}
\end{multicols}
\end{editorialboard} 


==> journaldata/SEC-journaldata.tex <==
\definecolor{bananayellow}{rgb}{1.0, 0.88, 0.21}
\colorlet{SECcolor}{bananayellow}   %new color names can be defined before use
\journalcolor      {SECcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Privacy and Security}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SEC}
\journalurl        {http://nowpublishers.com/SEC}
\journalissnprint  {2474-1558}
\journalissnonline {2474-1566}
\journaldoi        {10.1561/33}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
 Privacy and Security publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
\footnotesize
 \begin{itemize}
\item{Access control}
\item{Accountability}
\item{Anonymity}
\item{Application security}
\item{Artifical intelligence methods in security and privacy}
\item{Authentication}
\item{Big data analytics and privacy}
\item{Cloud security}
\item{Cyber-physical systems security and privacy}
\item{Distributed systems security and privacy}
\item{Embedded systems security and privacy}
\item{Forensics}
\item{Hardware security}
\item{Human factors in security and privacy}
\item{Information flow}
\item{Intrusion detection}
\item{Malware}
\item{Metrics}
\item{Mobile security and privacy}
\item{Language-based security and privacy}
\item{Network security}
\item{Privacy-preserving systems}
\item{Protocol security}
\item{Security and privacy policies}
\item{Security architectures}
\item{System security}
\item{Web security and privacy}
\end{itemize}
\normalsize
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Privacy and Security, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/SEC-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Hardware Platform Security for Mobile Devices}\\
Lachlan J. Gunn, N. Asokan, Jan-Erik Ekberg, Hans Liljestrand, Vijayanand Nayani and Thomas Nyman\\
ISBN: 978-1-68083-976-0\\
\\
\noindent \textit{Cloud Computing Security: Foundations and Research Directions}\\
Anrin Chakraborti, Reza Curtmola, Jonathan Katz, Jason Nieh, Ahmad-Reza Sadeghi, Radu Sion and Yinqian Zhang\\
ISBN: 978-1-68083-958-6\\
\\
\noindent \textit{Expressing Information Flow Properties}\\
Elisavet Kozyri, Stephen Chong and Andrew C. Myers\\
ISBN: 978-1-68083-936-4\\
\\
\noindent \textit{Accountability in Computing: Concepts and Mechanisms}\\
Joan Feigenbaum, Aaron D. Jaggard and Rebecca N. Wright\\
ISBN: 978-1-68083-784-1\\
\\
\noindent \textit{A Pragmatic Introduction to Secure Multi-Party Computation}\\
David Evans, Vladimir Kolesnikov and Mike Rosulek\\
ISBN: 978-1-68083-508-3\\
\\



==> journaldata/SIG-editorialboard.tex <==
%SIG-Editorialboard.

\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Yonina Eldar}{Weizmann Institute\\Israel}



\subsection{Editors}
\begin{multicols}{3}\raggedcolumns
\journaleditor{Pao-Chi Chang}{National Central University}
\journaleditor{Pamela Cosman}{University of California, San Diego}
\journaleditor{Michelle Effros}{California Institute of Technology}
\journaleditor{Yariv Ephraim}{George Mason University}
\journaleditor{Alfonso Farina}{Selex ES}
\journaleditor{Georgios Giannakis}{University of Minnesota}
\journaleditor{Vivek Goyal}{Boston University}
\journaleditor{Christine Guillemot}{INRIA}
\journaleditor{Sinan Gunturk}{New York University}
\journaleditor{Robert W. Heath, Jr.}{North Carolina State University}
\journaleditor{Sheila Hemami}{Triple Ring Technologies}
\journaleditor{Lina Karam}{Lebanese American University}
\journaleditor{Nick Kingsbury}{University of Cambridge}
\journaleditor{Alex Kot}{Nanyang Technical University}
\journaleditor{Jelena Kovacevic}{New York University}
\journaleditor{Geert Leus}{TU Delft}
\journaleditor{Jia Li}{Pennsylvania State University}
\journaleditor{Henrique Malvar}{Microsoft Research}
\journaleditor{B.S. Manjunath}{University of California, Santa Barbara}
\journaleditor{Urbashi Mitra}{University of Southern California}
\journaleditor{Bj\"{o}rn Ottersten}{KTH Stockholm}
\journaleditor{Vincent Poor}{Princeton University}
\journaleditor{Anna Scaglione}{Cornell Tech}
\journaleditor{Nicholas D. Sidiropoulos}{University of Virginia}
\journaleditor{Michael Unser}{EPFL}
\journaleditor{P.P. Vaidyanathan}{California Institute of Technology}
\journaleditor{Mihaela van der Shaar}{University of California, Los Angeles}
\journaleditor{Rabab Ward}{University of British Columbia}
\journaleditor{Ami Wiesel}{The Hebrew University of Jerusalem}
\journaleditor{Min Wu}{University of Maryland}
\journaleditor{Josiane Zerubia}{INRIA}
\end{multicols}
\end{editorialboard} 


==> journaldata/SIG-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{SIGcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {SIGcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Signal Processing}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SIG}
\journalurl        {http://www.nowpublishers.com/SIG}
\journalissnprint  {1932-8346}
\journalissnonline {1932-8354}
\journaldoi        {10.1561/20}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Signal Processing publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
\footnotesize
 \begin{itemize}
\item{Adaptive signal processing}
\item{Audio signal processing}
\item{Biological and biomedical signal processing}
\item{Complexity in signal processing}
\item{Digital signal processing}
\item{Distributed and network signal processing}
\item{Image and video processing}
\item{Linear and nonlinear filtering}
\item{Multidimensional signal processing}
\item{Multimodal signal processing}
\item{Multirate signal processing}
\item{Multiresolution signal processing}
\item{Nonlinear signal processing}
\item{Randomized algorithms in signal processing}
\item{Sensor and multiple source signal processing, source separation}
\item{Signal decompositions, subband and transform methods, sparse representations}
\item{Signal processing for communications}
\item{Signal processing for security and forensic analysis, biometric signal processing}
\item{Signal quantization, sampling, analog-to-digital conversion, coding and compression}
\item{Signal reconstruction, digital-to-analog conversion, enhancement, decoding and inverse problems}
\item{Speech/audio/image/video compression}
\item{Speech and spoken language processing}
\item{Statistical/machine learning}
\item{Statistical signal processing}
	\begin{itemize}
	\item{Classification and detection}
	\item{Estimation and regression}
	\item{Tree-structured methods}
	\end{itemize}
\end{itemize}
\normalsize
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Signal Processing, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/SIG-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Bilevel Methods for Image Reconstruction}\\
Caroline Crockett and Jeffrey A. Fessler\\
ISBN: 978-1-63828-002-6\\
\\
\noindent \textit{Operating Characteristics for Classical and Quantum Binary Hypothesis Testing}\\
Catherine A. Medlock and Alan V. Oppenheim\\
ISBN: 978-1-68083-882-4\\
\\
\noindent \textit{Foundations of User-Centric Cell-Free Massive MIMO}\\
Özlem Tugfe Demir, Emil Björnson and Luca Sanguinetti\\
ISBN: 978-1-68083-790-2\\
\\
\noindent \textit{Data-Driven Multi-Microphone Speaker Localization on Manifolds}\\
Bracha Laufer-Goldshtein, Ronen Talmon and Sharon Gannot\\
ISBN: 978-1-68083-736-0\\
\\
\noindent \textit{Recent Advances in Clock Synchronization for Packet-Switched Networks}\\
Anantha K. Karthik and Rick S. Blum\\
ISBN: 978-1-68083-726-1\\


==> journaldata/STP-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Albert N. Link}{University of North Carolina at Greensboro\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{David Audretsch}{Indiana University}
\journaleditor{William Bonvillian}{MIT}
\journaleditor{Barry Bozeman}{Arizona State University}
\journaleditor{Kaye Husbands Fealing}{Georgia Institute of Technology}
\journaleditor{John Hardin}{North Carolina Board of Science and Technology}
\journaleditor{Mariagrazia Squicciarini}{OECD}
\journaleditor{Wolfgang Polt}{Joanneum Research Institute}
\journaleditor{Nicholas Vonortas}{The George Washington University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/STP-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{ASTPcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {ASTPcolor} %a color name. 
\journaltitle      {Annals of Science and Technology Policy}
%\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ASTP}
\journalurl        {http://www.nowpublishers.com/ASTP}
\journalissnprint  {2475-1820}
\journalissnonline {2475-1812}
\journaldoi        {10.1561/110}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Annals of Science and Technology Policy publishes
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Literature reviews of technology and innovation policies}
\item{Historical case studies of technology development and implementation}
\item{Institutional histories of technology- and innovation-based organizations}
\item{Analyses of policies attendant to technology development and adoption and diffusion}
\item{Studies documenting the adoption and diffusion of technologies and subsequent consequences}
\item{Studies of public and private research partnerships (cross sectional, over time, or case based)}
\item{Assessments and evaluations of specific technology and innovation policies}
\item{Analyses of ecosystems associated with the technology and/or innovation development}
\item{Cross observational (e.g., cross-agency or cross-country) comparisons of technology and innovation policies}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
  Annals of Science and Technology Policy, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/SYS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Panos J. Antsaklis}{University of Notre Dame\\United States}
\journalchiefeditor{Alessandro Astolfi}{Imperial College London, United Kingdom\\ University of Rome ''Tor Vergata'', Italy}



\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{John Baillieul}{Boston University}
\journaleditor{Peter Caines}{McGill University}
\journaleditor{Christos Cassandras}{Boston University}
\journaleditor{Denis Dochain}{UC Louvain}
\journaleditor{Magnus Egerstedt}{Georgia Institute of Technology}
\journaleditor{Karl Henrik Johansson}{KTH Stockholm}
\journaleditor{Miroslav Krstic}{University of California, San Diego}
\journaleditor{Jan Maciejowski}{University of Cambridge}
\columnbreak
\journaleditor{Dragan Nesic}{The University of Melbourne}
\journaleditor{Marios Polycarpou}{University of Cyprus}
\journaleditor{J\"{o}rg Raisch}{Technical University Berlin}
\journaleditor{Arjan van der Schaft}{University of Groningen}
\journaleditor{M. Elena Valcher}{University of Padova}
\journaleditor{Richard Vinter}{Imperial College London}
\journaleditor{George Weiss}{Tel Aviv University}
\end{multicols*}
\end{editorialboard} 

==> journaldata/SYS-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet {SYScolor}{cobalt} %new color names can be defined before use
\journalcolor      {SYScolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Systems and Control}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SYS}
\journalurl        {http://www.nowpublishers.com/SYS}
\journalissnprint  {2325-6818}
\journalissnonline {2325-6826}
\journaldoi        {10.1561/26}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Systems and Control publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Control of:}
	\begin{itemize}
	\item{Hybrid and Discrete Event Systems}
	\item{Nonlinear Systems}
	\item{Network Systems}
	\item{Stochastic Systems}
	\item{Multi-agent Systems}
	\item{Distributed Parameter Systems}
	\item{Delay Systems}
	\end{itemize}
	\columnbreak
\item{Filtering, Estimation, Identification}
\item{Optimal Control}
\item{Systems Theory}
\item{Control Applications}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Systems and Control, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/SYS-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Finite-Time Stability Tools for Control and Estimation}\\
Denis Efimov and Andrey Polyakov\\
ISBN: 978-1-68083-926-5\\
\\
\noindent \textit{Generalized Coordination of Multi-robot Systems}\\
Kazunori Sakurama and Toshiharu Sugie\\
ISBN: 978-1-68083-902-9\\
\\
\noindent \textit{Analysis and Control for Resilience of Discrete Event Systems: Fault Diagnosis, Opacity and Cyber Security}\\
João Carlos Basilio, Christoforos N. Hadjicostis and Rong Su\\
ISBN: 978-1-68083-856-5\\
\\
\noindent \textit{Learning-Based Control: A Tutorial and Some Recent Results}\\
Zhong-Ping Jiang, Tao Bian and Weinan Gao\\
ISBN: 978-1-68083-752-0\\
\\
\noindent \textit{Synchronous Reinforcement Learning-Based Control for Cognitive Autonomy}\\
Kyriakos G. Vamvoudakis and Nick-Marios T. Kokolakis\\
ISBN: 978-1-68083-744-5\\
\\
\noindent \textit{Achieving Ecological Resilience Through Regime Shift Management}\\
M. D. Lemmon\\
ISBN: 978-1-68083-716-2\\



==> journaldata/TCS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Salil Vadhan}{Harvard University\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Bernard Chazelle}{Princeton University}
\journaleditor{Oded Goldreich}{Weizmann Institute}
\journaleditor{Shafi Goldwasser}{Massachusetts Institute of Technology and Weizmann Institute}
\journaleditor{Sanjeev Khanna}{University of Pennsylvania}
\journaleditor{Jon Kleinberg}{Cornell University}
\journaleditor{L\'aszl\'o Lov\'asz}{Eötvös Lor\'and University}
\journaleditor{Christos Papadimitriou}{University of California, Berkeley}
\journaleditor{Peter Shor}{Massachusetts Institute of Technology}
\journaleditor{Eva Tardos}{Cornell University}
\journaleditor{Avi Wigderson}{AIS, Princeton University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/TCS-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{TCScolor}{cobalt}   %new color names can be defined before use
\journalcolor      {TCScolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Theoretical Computer Science}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {TCS}
\journalurl        {http://www.nowpublishers.com/TCS}
\journalissnprint  {1551-305X}
\journalissnonline {1551-3068}
\journaldoi        {10.1561/04}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in Theoretical Computer Science publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Algorithmic game theory}
    \item{Computational algebra}
    \item{Computational aspects of combinatorics and graph theory}
    \item{Computational aspects of communication}
    \item{Computational biology}
    \item{Computational complexity}
    \item{Computational geometry}
    \item{Computational learning}
    \item{Computational Models and Complexity}
    \item{Computational Number Theory}
    \item{Cryptography and information security}
    \item{Data structures}
    \item{Database theory}
    \item{Design and analysis of algorithms}
    \item{Distributed computing}
    \item{Information retrieval}
    \item{Operations Research}
    \item{Parallel algorithms}
    \item{Quantum Computation}
    \item{Randomness in Computation}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in Theoretical Computer Science, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/TCS-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Complexity Theory, Game Theory, and Economics: The Barbados Lectures}\\
Tim Roughgarden\\
ISBN: 978-1-68083-654-7\\
\\
\noindent \textit{Semialgebraic Proofs and Efficient Algorithm Design}\\
Noah Fleming, Pravesh Kothari and Toniann Pitassi\\
ISBN: 978-1-68083-636-3\\
\\
\noindent \textit{Higher-order Fourier Analysis and Applications}\\
Hamed Hatami, Pooya Hatami and Shachar Lovett\\
ISBN: 978-1-68083-592-2\\
\\
\noindent \textit{On Doubly-Efficient Interactive Proof Systems}\\
Oded Goldreich \\
ISBN: 978-1-68083-424-6\\
\\
\noindent \textit{Coding for Interactive Communication: A Survey}\\
Ran Gelles\\
ISBN: 978-1-68083-346-1\\

==> journaldata/TOM-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Panos Kouvelis}{Washington University St. Louis\\USA}

\subsection{Editors}
\journaleditor{Charles Corbett}{UCLA, USA}
\journaleditor{Uday Karmarkar}{UCLA, USA}

\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Onur Bayabatli}{Singapore Management University, Singapore}
\journaleditor{Jan Fransoo}{Tilburg University, The Netherlands} 
\journaleditor{Chuck Munson}{Washington State University, USA} 
\journaleditor{Nicholas Petruzzi}{Pennsylvania State University, USA}
\journaleditor{Guillaume Roels}{INSEAD, France}
\journaleditor{Nicola Secomandi}{Carnegie-Mellon University, USA} 
\journaleditor{Zuo-Jun Max Shen}{University of California, Berkeley, USA} 
\journaleditor{Sherri Xiaole Wu}{Fudan University, China} 
\journaleditor{Y. Karen Zheng}{MIT, USA} 
%\end{multicols*}
\end{editorialboard} 

==> journaldata/TOM-journaldata.tex <==
\definecolor{cerise}{rgb}{0.87, 0.19, 0.39}
\colorlet{TOMcolor}{cerise}   %new color names can be defined before use
\journalcolor      {TOMcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Technology, Information and Operations Management}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {TOM}
\journalurl        {http://www.nowpublishers.com/TOM}
\journalissnprint  {1571-9545}
\journalissnonline {1571-9553}
\journaldoi        {10.1561/02}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Technology, Information and Operations Management publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{B2B Commerce}
\item{Business Process Engineering and Design}
\item{Business Process Outsourcing}
\item{Capacity Planning}
\item{Competitive Operations}
\item{Contracting in Supply Chains}
\item{E-Commerce and E-Business Models}
\item{Electronic markets, auctions and exchanges}
\item{Enterprise Management Systems}
\item{Facility Location}
\item{Information Chain Structure and Competition}
\item{International Operations}
\item{Marketing/Manufacturing Interfaces}
\item{Multi-location inventory theory}
\item{New Product \& Service Design}
\item{Queuing Networks}
\item{Reverse Logistics}
\item{Service Logistics and Product Support}
\item{Supply Chain Management}
\item{Technology Management and Strategy}
\item{Technology, Information and Operations in:}
	\begin{itemize}
	\item{Automotive Industries}
	\item{Electronics manufacturing}
	\item{Financial Services}
	\item{Health Care}
	\item{Media and Entertainment}
	\item{Process Industries}
	\item{Retailing}
	\item{Telecommunications}
	\end{itemize}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Technology, Information and Operations Management, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/TOM-seriespage.tex <==
\vspace{12pt}
\noindent \textit{The Interface of Finance, Operations, and Risk Management}\\
Volodymyr Babich and John R. Birge
\\ISBN: 978-1-68083-796-4
\\
\\
\noindent \textit{AI and Business Models: The Good, The Bad and The Ugly}\\
Vania Sena and Manuela Nocker
\\ISBN: 978-1-68083-794-0
\\
\\
\noindent \textit{The Business of Electric Vehicles: A Platform Perspective}\\
Jonas Boehm, Hemant K. Bhargava and Geoffrey G. Parker
\\ISBN: 978-1-68083-762-9
\\
\\
\noindent \textit{Advances in Supply Chain Finance and FinTech Innovations Overview}\\
Panos Kouvelis, Ling Dong and Danko Turcic
\\ISBN: 978-1-68083-722-3

==> journaldata/WEB-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\begin{multicols}{1}%\raggedcolumns
\journalchiefeditor{Wendy Hall}{University of Southampton, UK}
\journalchiefeditor{Noshir R. Contractor}{Northwestern University, USA}
\journalchiefeditor{Kieron O'Hara}{University of Southampton, UK}
\end{multicols}

\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Tim Berners-Lee}{Massachusetts Institute of Technology}
\journaleditor{Noshir Contractor}{Northwestern University}
\journaleditor{Lorrie Crano}{Carnegie Mellon University}
\journaleditor{Dieter Fensel}{University of Innsbruck}
\journaleditor{Carole Goble}{University of Manchester}
\journaleditor{Pat Hayes}{IHMC}
\journaleditor{James Hendler}{Rensselaer Polytechnic Institute}
\journaleditor{Arun Iyengar}{IBM Research}
%\columnbreak
\journaleditor{Craig Knoblock}{University of Southern California}
\journaleditor{Ora Lassila}{Pegasystems}
\journaleditor{Sun Maosong}{Tsinghua University}
\journaleditor{Cathy Marshall}{Microsoft}
\journaleditor{Peter Monge}{University of Southern California}
\journaleditor{Ben Shneiderman}{University of Maryland}
\journaleditor{Danny Weitzner}{Massachusetts Institute of Technology}
\journaleditor{Yorick Wilks}{University of Sheffield}
\end{multicols*}
\end{editorialboard} 

==> journaldata/WEB-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{WEBcolor}{brickred}   %new color names can be defined before use
\journalcolor      {WEBcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Web Science}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {WEB}
\journalurl        {http://www.nowpublishers.com/WEB}
\journalissnprint  {1551-3939}
\journalissnonline {1551-3947}
\journaldoi        {10.1561/10}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Web Science publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Agents and the Semantic Web}
    \item{Collective Intelligence}
    \item{Content Management}
    \item{Databases on the Web}
    \item{Data Mining}
    \item{Democracy and the Web}
    \item{Dependability}
    \item{Economics of information and the Web}
    \item{E-Crime}
    \item{E-Government}
    \item{Emergent behaviour}
    \item{Ethics}
    \item{Hypertext/Hypermedia}
    \item{Identity}
    \item{Languages on the Web}
    \item{Memories for Life}
    \item{Mobile/Pervasive}
    \item{Network Infrastructures}
    \item{Performance}
    \item{Privacy}
    \item{Scalability}
    \item{Security}
    \item{Semantic Web}
    \item{Social Networking}
    \item{Standards}
    \item{The Law and the Web}
    \item{The Web as an Educational Tool}
    \item{The Web in the Developing World}
    \item{Trust and Provenance}
    \item{Universal Usability}
    \item{User Interfaces}
    \item{Virtual Reality}
    \item{Web Art}
    \item{Web Governance}
    \item{Search}
    \item{Web Services}
\end{itemize}
\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Web Science, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/WEB-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Tracking on the Web, Mobile and the Internet of Things}\\
Reuben Binns\\
ISBN: 978-1-68083-964-7\\
\\
\noindent \textit{Inclusive Security: Digital Security Meets Web Science}\\
Lizzie Coles-Kemp\\
ISBN: 978-1-68083-782-7\\
\\
\noindent \textit{An Introduction to Hybrid Human-Machine Information Systems}\\
Gianluca Demartini, Djellel Eddine Difallah, Ujwal Gadiraju and\\ Michele Catasta\\
ISBN: 978-1-68083-374-4\\
\\
\noindent \textit{Minds Online: The Interface between Web Science, Cognitive Science and the Philosophy of Mind}\\
Paul Smart, Robert Clowes and Richard Heersmink\\
ISBN: 978-1-68083-322-5\\
\\
\noindent \textit{Collective Attention on the Web}\\
Christian Bauckhage and Kristian Kersting\\
ISBN: 978-1-68083-204-4
